Theoretical and computational analysis of the thermal quasi-geostrophic model

This work involves theoretical and numerical analysis of the Thermal Quasi-Geostrophic (TQG) model of submesoscale geophysical fluid dynamics (GFD). Physically, the TQG model involves thermal geostrophic balance, in which the Rossby number, the Froude number and the stratification parameter are all of the same asymptotic order. The main analytical contribution of this paper is to construct local-in-time unique strong solutions for the TQG model. For this, we show that solutions of its regularized version $\alpha$-TQG converge to solutions of TQG as its smoothing parameter $\alpha \rightarrow 0$ and we obtain blowup criteria for the $\alpha$-TQG model. The main contribution of the computational analysis is to verify the rate of convergence of $\alpha$-TQG solutions to TQG solutions as $\alpha \rightarrow 0$ for example simulations in appropriate GFD regimes.

==> Kato Existence/numerics.tex <==
\section{Numerical implementation}\label{sec: numerics}
% \ADD{todo: add references}
{For numerical implementation, we choose to work in weaker spaces than what the wellposedness theorem dictates. Additionally we allow for boundary conditions in the numerical setup. We recognise these choices create gaps between the theory and the implementation.}

\subsection{Discretisation methods for $\alpha$--TQG and TQG   }\label{sec: numerics methods}

In this subsection, we describe the finite element (FEM) spatial discretisation, and finite difference Runge-Kutta time stepping discretisation methods that are utilised for the $\alpha$-TQG system. 
By setting $\alpha$ to zero we obtain our numerical setup for the TQG system. 

Consider a bounded domain $\domain$. Let $\p \domain$ denote the boundary. We impose Dirichlet boundary conditions
\begin{equation}\label{eq: tqg boundary conditions numerical}
    \psi^\alpha = 0, \    
    \Delta \psi^\alpha = 0, \qquad \text{on } \p \domain.
\end{equation}
For $\domain = \mathbb T^2$, our numerical setup does not change, in which case the boundary flux terms in the discretised equations are set to zero.

\subsubsection{The stream function equation}\label{sec: stream function discretisation}

Let $H^{1}\left(\domain\right)$ denote the Sobolev $W^{1,2}\left(\domain\right)$
space and let $\left\Vert .\right\Vert _{\partial\domain}$ denote
the $L^{2}\left(\partial\domain\right)$ norm. 
Define the space 
\begin{equation}\label{eq: w1 space}
    W^{1}\left(\domain\right):=\left\{ \nu\in H^{1}\left(\domain\right)\left|\left\Vert \nu\right\Vert _{\partial\domain}=0\right.\right\}.
\end{equation}
We express \eqref{constrtAlpha} as two inhomogeneous Helmholtz equations
\begin{align}
    \omega^\alpha - f &= (\Delta -1 ) \tilde\psi \label{eq:inhomogeneousHelmholtz}\\
    -\tilde\psi &= (\alpha \Delta - 1)\psi^\alpha\label{eq:inhomogeneousHelmholtzAlpha}. 
\end{align}
We take $\tilde\psi,\psi^\alpha \in W^1 (\domain)$.
Since the two equations are of the same form, let us first consider \eqref{eq:inhomogeneousHelmholtz}.
Using an arbitrary test function $\phi \in W^1(\domain)$, we obtain the following weak form of \eqref{eq:inhomogeneousHelmholtz},
\begin{align}
\langle\nabla \tilde\psi,\nabla\phi\rangle_\domain +\langle\tilde\psi,\phi\rangle_\domain  &=  -\langle \omega^\alpha - f, \phi \rangle_\domain.
\label{eq: inhomogeneousHelmholtz weak}
\end{align}
Define the functionals
\begin{align}
    L_\alpha(v, \phi) &:= \alpha\langle \nabla v, \nabla \phi \rangle_\domain +\langle v, \phi  \rangle_\domain \label{eq: psi bilinear form}\\
    F_{\cdot}(\phi) &:=  -\langle  \cdot, \phi \rangle_\domain
    \label{eq: psi linear form}
\end{align}
for $v, \phi \in W^1(\domain)$, then \eqref{eq: inhomogeneousHelmholtz weak} can be written as
\begin{equation}\label{eq: TQG weak elliptic}
    L_1(\tilde\psi, \phi) = F_{\omega^\alpha -  f^\alpha}(\phi).
\end{equation}
And similarly for \eqref{eq:inhomogeneousHelmholtzAlpha}, we have
\begin{equation}\label{eq: TQG weak elliptic alpha} 
    L_\alpha(\psi^\alpha, \phi) = F_{-\tilde\psi}(\phi).
\end{equation}
We discretise equations \eqref{eq: TQG weak elliptic} and \eqref{eq: TQG weak elliptic alpha} using a continuous
Galerkin (CG) discretisation scheme. 

Let $\delta$ be the discretisation parameter, and let $\domain_\delta$ denote a space filling triangulation of the domain, that consists of geometry-conforming nonoverlapping elements.
%Let $X_\delta^k$ denote the finite element space that consists of continuous functions, and including at least all polynomials of degree $k$ on each cell of $\domain_\delta$. 
Define the approximation space
% \begin{equation}
%     W^k_\delta = W^1(\domain) \cap X_\delta^k
% \end{equation}
% where $X_\delta^k$ is a finite element space consisting of continuous functions and including at least all polynomials of degree $k$ on each element of a triangulation $\domain_\delta$. More specifically, we have 
\begin{equation} \label{eq: cg space}
    W_\delta^{k}(\domain):=\left\{ \phi_\delta\in W^{1}\left(\domain\right)\ : \ \phi_\delta\in C\left(\domain\right),\left.\phi_\delta\right|_{K}\in\Pi^{k}\left(K\right)\text{ each } K \in \domain_\delta\right\}.
\end{equation}
in which $C(\domain)$ is the space of continuous functions on $\domain$, and  $\Pi^{k}\left(K\right)$ denotes the space of polynomials of degree at most $k$ on element $K\in \domain_\delta$. 

For \eqref{eq: TQG weak elliptic}, given $f_\delta \in W_\delta^k(\domain)$ and $\omega_\delta \in V_\delta^k(\domain)$ (see \eqref{DG space} for the definition of $V_\delta^k(\domain)$), 
our numerical approximation is the solution $\tilde\psi_\delta \in W_\delta^k(\domain)$ that satisfies 
\begin{equation}
L_1(\tilde\psi_\delta, \phi_\delta) = F_{\omega_\delta - f_\delta}(\phi_\delta)
\label{eq: TQG psi eqn weak discretised}
\end{equation}
for all test functions $\phi_\delta \in W_\delta^k(\domain)$. Then, using $\tilde\psi_\delta$, our numerical approximation of $\psi^\alpha$ is the solution $\psi_\delta^\alpha\in W_\delta^k(\domain)$ that satisfies
\begin{equation}\label{eq: TQG psi alpha eqn weak discretised}
L_\alpha(\psi_\delta^\alpha, \phi_\delta) = F_{-\tilde\psi_\delta} (\phi_\delta)
\end{equation}
for all test functions $\phi_\delta \in W_\delta^k(\domain)$.

 For a detailed exposition of the numerical algorithms that solves the discretised problems \eqref{eq: TQG psi eqn weak discretised} and \eqref{eq: TQG psi alpha eqn weak discretised} we point the reader to \cite{Gibson2019, Brenner2008}.

\subsubsection{Hyperbolic equations}\label{sec: buoyancy equation discretisation}
We choose to discretise the hyperbolic buoyancy \eqref{ceAlpha} and potential vorticity \eqref{meAlpha} equations using a discontinuous Galerkin (DG) scheme. For a detailed exposition of DG methods, we refer the interested reader to \cite{Hesthaven2008}.

Define the DG approximation space, denoted by $V_\delta^k(\domain)$, to be the element-wise polynomial space,
\begin{equation}\label{DG space}
    V_\delta^k(\domain) = \left\{ \left. v_\delta \in L^2(\domain) \right|\forall K \in \domain_\delta,\ \exists\phi_\delta\in \Pi^k (K):\ \left.v_\delta\right|_{K}=\left.\phi_\delta\right|_K\right\}.
\end{equation}
We look to approximate $b^\alpha$ and $\omega^\alpha$ in the space $V_\delta^k(\domain)$. Essentially, this means our approximations of $b^\alpha$ and $\omega^\alpha$ are each an direct sum over the elements in $\domain_\delta$. Additional constraints on the numerical fluxes across shared element boundaries are needed to ensure conservation properties and stability. 
Further, note that $W^k_\delta(\domain) \subset V^k_\delta(\domain)$. This inclusion is also needed for ensuring numerical conservation laws, see Section \ref{sec: numerics numerical conservation}.

For the buoyancy equation \eqref{ceAlpha}, we obtain the following variational formulation
\begin{align}
\langle \p_t b^\alpha, \nu_\delta \rangle _{K} & = \langle b^\alpha {\bf u}^\alpha,\nabla\nu_\delta\rangle _K - \langle b^\alpha {\bf u}^\alpha\cdot\normal,\nu_\delta\rangle _{\partial K},\quad K\in \domain_\delta
\label{eq: TQG b alpha equation weak}
\end{align}
where $\nu_\delta\in V^k_\delta(\domain)$ is any test function, $\p K$ denotes the boundary of $K$, and $\normal$ denotes the unit normal vector to $\p K$. Let $b^\alpha_\delta$ be the approximation of $b^\alpha$ in $V_\delta^k$, and let $\bu^\alpha_\delta = \nabla^\perp \psi^\alpha_\delta$ for $\psi^\alpha_\delta \in W^k_\delta$. Our discretised buoyancy equation over each element is given by
\begin{equation}
    \langle \p_t b^\alpha_\delta, \nu_\delta \rangle _{K} = \langle b^\alpha_\delta{\bf u}^\alpha_\delta,\nabla\nu_\delta\rangle _K - \langle b^\alpha_\delta{\bf u}^\alpha_\delta \cdot \normal,\nu_\delta\rangle _{\partial K}, \quad K \in \domain_\delta.
    \label{eq: TQG b alpha eqn weak discretised}
\end{equation}

Similarly, let $\omega^\alpha_\delta \in V_\delta^k(\domain)$ be the approximation of $\omega^\alpha$, and let $h_\delta \in W_\delta^k$. We obtain the following discretised variational formulation that corresponds to \eqref{meAlpha}, 
\begin{align}
\langle \p_t \omega^\alpha_\delta, \nu_\delta \rangle _{K} 
&= \langle (\omega^\alpha_\delta - b^\alpha_\delta){\bf u}^\alpha_\delta,\nabla\nu_\delta\rangle _{K}
-\langle (\omega^\alpha_\delta - b^\alpha_\delta) {\bf u}^\alpha_\delta \cdot\normal,\nu_\delta\rangle _{\partial K} \nonumber \\
& \qquad - \frac12\langle \nabla \cdot (b^\alpha_\delta \nabla^\perp h_\delta), \nu_\delta \rangle _K,
\qquad K\in \domain_\delta,
\label{eq: TQG omega alpha eqn weak discretised}
\end{align}
for test function $\nu_\delta \in V_\delta^k(\domain)$. 
% \begin{align}
% \langle\p_{t}\omega_\delta^\alpha,\nu_\delta
% \rangle_{K} 
% & =
% \langle(\omega^\alpha_\delta - b^\alpha_\delta) \nabla^{\perp} \psi_\delta,\nabla\nu_\delta\rangle_{K}-\langle\hat{f}_{\omega}(\omega_\delta^{+},\omega_\delta^{-},\nabla^{\perp}\psi_\delta\cdot\hat{n}),\nu_\delta^{-}\rangle_{\partial K}\nonumber \\
%  & \qquad-\frac{1}{2}\langle\nabla\cdot(b_\delta\nabla^{\perp}\rmh_\delta),\nu_\delta\rangle_{K}
% \label{eq: TQG omega eqn weak discretised}
% \end{align}

At this point, we only have the discretised problem on single elements. To obtain the global approximation, we sum over all the elements in $\domain_\delta$. In doing so, the $\p K$ terms in \eqref{eq: TQG b alpha eqn weak discretised} and \eqref{eq: TQG omega alpha eqn weak discretised} must be treated carefully.
Let $\p K_\text{ext}$ denote the part of cell boundary that is contained in $\p \domain$. Let $\p K_\text{int}$ denote the part of the cell boundary that is contained in the interior of the domain $\domain\backslash \p \domain$.
On $\p K_\text{ext}$ we simply impose the PDE boundary conditions. However, on $\p K_\text{int}$ we need to consider the contribution from each of the neighbouring elements.
By choice, the approximant $\psi^\alpha_\delta \in W_\delta^k$ is continuous on $\p K$. And since
\begin{equation}
    \bu^\alpha_\delta \cdot \normal = \nabla^\perp \psi^\alpha_\delta \cdot \normal = -\nabla \psi^\alpha_\delta \cdot \hat \tau = -\frac{\dd\psi^\alpha_\delta}{\dd\hat\tau},
\end{equation}
where $\hat\tau$ denotes the unit tangential vector to $\p K$, $\bu^\alpha_\delta \cdot \normal$ is also continuous. This means  $\bu^\alpha_\delta \cdot \normal$ in \eqref{eq: TQG b alpha eqn weak discretised} (also in \eqref{eq: TQG omega alpha eqn weak discretised}) is single valued. However, due to the lack of global continuity constraint in the definition of $V_k^\alpha(\domain)$, $b^\alpha_\delta$ and $\omega^\alpha_\delta$ are multi-valued on $\p K_\text{int}$. Thus, as our approximation of $\omega^\alpha$ and $b^\alpha$ over the whole domain is the sum over $K \in \domain_\delta$,  we have to constrain the flux on the set $\left(\bigcup_{K\in\domain_\delta} \p K \right)\setminus \p \domain$. This is done using appropriately chosen numerical flux fields in the boundary terms of \eqref{eq: TQG b alpha eqn weak discretised} and \eqref{eq: TQG omega alpha eqn weak discretised}.

Let 
{$\nu^{-}:=\lim_{\epsilon\uparrow0} \nu ({\bf x}+\epsilon\normal)$} 
and 
{ $\nu^{+}:=\lim_{\epsilon\downarrow0}\nu ({\bf x}+\epsilon\normal)$}, 
for ${\bf x}\in\partial K$, be the inside and outside (with respect to a fixed element $K$) values respectively, of a function $\nu$ on the boundary.
Let $\hat{f}$ be a \emph{numerical flux} function 
that satisfies the following properties:
\begin{enumerate}[(i)]
    \item consistency 
    \begin{equation}
     \hat f (\nu, \nu, \bu_\delta \cdot \normal) = \nu \bu_\delta\cdot\normal
     \label{eq: nflux consistency}
     \end{equation}
    
    \item conservative
    \begin{equation}
        \hat f (\nu^+, \nu^-, \bu_\delta\cdot \normal) = - \hat f (\nu^-, \nu^+, -\bu_\delta\cdot \normal)
        \label{eq: nflux conservative}
    \end{equation}
    
    \item $L^2$ stable in the enstrophy norm with respect to the buoyancy equation, see \cite[Section 6]{Bernsen2006}.
\end{enumerate}
% \CHANGE{Upwind scheme
% \[
% \hat{f} (b_\delta^{+},b_\delta^{-},{\bf u}\cdot\hat{n} )={\bf u}\cdot\hat{n}\begin{cases}
% b_\delta^{+} & \text{if }{\bf u}\cdot\hat{n}<0\\
% b_\delta^{-} & \text{if }{\bf u}\cdot\hat{n}\geq0.
% \end{cases}
% \]}
With such an $\hat f$, we replace 
$b^\alpha_\delta \bu^\alpha_\delta \cdot \normal$ by the numerical flux $\hat{f}(b_\delta^{\alpha, +},b_\delta^{\alpha, -},{\bf u}^\alpha_\delta \cdot\normal)$  in \eqref{eq: TQG b alpha eqn weak discretised}.
Similarly, in \eqref{eq: TQG omega alpha eqn weak discretised}, we replace $(\omega^\alpha_\delta - b^\alpha_\delta)\bu_\delta^\alpha \cdot \normal$ by $\hat{f}((\omega^\alpha_\delta - b^\alpha_\delta)^{+}, (\omega^\alpha_\delta - b^\alpha_\delta)^{-}, \bu_\delta^\alpha \cdot \normal)$.

\begin{remark}
For a general nonlinear conservation law, one has to solve what is called the \emph{Riemann problem} for the numerical flux, see \cite{Hesthaven2008} for details.
In our setup, we use the following local Lax-Friedrichs flux, which is an approximate Riemann solver,
\begin{equation}
\hat{f}(\nu^+, \nu^-, \bu_\delta\cdot\normal) = \bu_\delta\cdot\normal
\{\{ \nu  \}\} - \frac{|\bu_\delta\cdot\normal|}{2}\llbracket\nu\rrbracket
\end{equation}
where
\begin{equation}
\{\{\nu\}\}:=\frac{1}{2}(\nu^{-}+\nu^{+}),\qquad
\llbracket\nu\rrbracket:=\normal^{-}\nu^{-}+\normal^{+}\nu^{+}.
\end{equation}
\end{remark}

Finally, our goal is to find $b^\alpha_\delta, \omega^\alpha_\delta \in V_\delta^k(\domain)$ such that for all {$\nu_\delta\in V_\delta^k(\domain)$} we have
\begin{align}
\sum_{K\in \domain_\delta} \langle \p_t b^\alpha_\delta, \nu_\delta\rangle _{K} 
&=
\sum_{K\in \domain_\delta}
\big\{
\langle b^\alpha_\delta\nabla^{\perp} \psi^\alpha_\delta, \nabla \nu_\delta\rangle _{K}  -
\langle \hat{f}_{b^\alpha}(b_\delta^{\alpha, +},b_\delta^{\alpha, -},\nabla^{\perp}\psi^\alpha_\delta \cdot \normal), \nu_\delta^{-}\rangle _{\partial K}
\big\}, 
\label{eq: TQG b eqn weak discretised numerical flux}
\\
\sum_{K\in \domain_\delta} \langle \p_t \omega^\alpha_\delta, \nu_\delta \rangle _{K} 
&= 
\sum_{K\in \domain_\delta} 
\big\{
\langle (\omega^\alpha_\delta - b^\alpha_\delta)\nabla^{\perp}\psi^\alpha_\delta,\nabla\nu_\delta\rangle _{K} - \frac12\langle \nabla \cdot (b^\alpha_\delta \nabla^\perp h_\delta), \nu_\delta \rangle _K
\label{eq: TQG omega eqn weak discretised numerical flux}
% \\
% &\qquad\quad
% -\langle \omega^\alpha_\delta \nabla^\perp \psi^\alpha_\delta \cdot\normal,
% \nu_\delta^-
% \rangle _{\partial K_\text{ext}}
% \nonumber
\\
&\qquad -
\langle \hat{f}_{\omega^\alpha}((\omega^\alpha_\delta - b^\alpha_\delta)^{+}, (\omega^\alpha_\delta - b^\alpha_\delta)^{-}, \nabla^\perp \psi_\delta^\alpha \cdot \normal),
\nu_\delta^ -
\rangle _{\partial K}
\big\}
\nonumber
\end{align}
with $\psi_\delta^\alpha \in W_\delta^k(\domain)$ being the numerical approximation to the stream function. 

\begin{remark}
In \eqref{eq: TQG b eqn weak discretised numerical flux} and \eqref{eq: TQG omega eqn weak discretised numerical flux} we do not explicitly distinguish $\p K_\text{ext}$ and $\p K_\text{int}$ because for the boundary conditions \eqref{eq: tqg boundary conditions numerical}, the $\p K_\text{ext}$ terms vanish. 
\end{remark}


\subsubsection{Numerical conservation}
\label{sec: numerics numerical conservation}
Conservation properties of the TQG system was first shown in \cite{Holm2021}. More specifically, the TQG system conserves energy, and an infinite family of quantities called casimirs. Proposition \ref{prop: TQG alpha conservation} below describes the conservation properties of the $\alpha$--TQG system. We note that the form of the conserved energy and casimirs are the same as that of the TQG system.
Although the result is stated for the system with boundary conditions, it is easy to show that the same result holds for $\mathbb T^2$ .

\begin{proposition}[$\alpha$--TQG conserved quantities]\label{prop: TQG alpha conservation}
On a bounded domain $\domain$ with boundary $\p \domain$, consider the $\alpha$-TQG system \eqref{ceAlpha} -- \eqref{constrtAlpha} 
with boundary conditions
\begin{equation}\label{eq: tqg boundary conditions}
    \normal\cdot \bu^\alpha = 0, \  \normal\times \nabla b^\alpha = 0,\   
    \frac \dd {\dd t}
    \int_{\p \domain} \nabla \psi^\alpha \cdot \normal = 0, \ 
    \frac \dd {\dd t}
    \int_{\p \domain}  \nabla \Delta \psi^\alpha \cdot \normal = 0, \ 
    \normal \times \nabla \Delta \psi^\alpha = 0
\end{equation}
We have
\begin{equation}\label{eq: tqg energy}
     E^\alpha(t) := - \frac12  \int_\domain \{(\omega^\alpha - f)\psi^\alpha + \rmh b^\alpha \} \dd \bx,
\end{equation}
and
\begin{equation}\label{eq: tqg casimirs}
     C^\alpha_{\Psi, \Phi}(t) :=   \int_\domain \{ \Psi(b^\alpha) + \omega^\alpha \Phi(b^\alpha) \} \dd \bx ,\qquad \forall \Psi, \Phi \in C^\infty
\end{equation}
are conserved, i.e. $\dd_t E^\alpha(t) = 0$ and $\dd_t C^\alpha_{\Psi, \Phi}(t) = 0$.
\end{proposition}

\begin{proof}
For the energy $E^\alpha(t)$, we obtain
\begin{align*}
    \frac \dd {\dd t} E^\alpha(t) &= -\frac12 \frac \dd {\dd t} \int_\domain \{\psi^\alpha (\Delta - 1)(1-\alpha \Delta)\psi^\alpha + \rmh b^\alpha \} \dd \bx \\
    % &= -\frac12 \int_\domain \{\p_t \psi (\Delta -1)(1-\alpha\Delta)\psi + \psi (\Delta-1)(1-\alpha\Delta)\p_t \psi + h \p_t b \} \dd \bx \\
    &=\int_\domain \{-\psi^\alpha \ \p_t \omega^\alpha - \frac12 h \p_t b^\alpha \} \dd\bx.
\end{align*}
Substitute $\p_t \omega^\alpha$ and $\p_t b^\alpha$ using \eqref{ceAlpha} and \eqref{meAlpha},
the result then follows from direct calculations.

Similarly for the casimirs, we obtain the result by directly evaluating $\dd_t C^\alpha_{\Psi, \Phi}(t)$.
\end{proof}

\begin{remark}
In \eqref{eq: tqg boundary conditions}, except for the integral Neumann boundary conditions, we effectively have Dirichlet boundary conditions for $\psi^\alpha$, $b^\alpha$ and $\Delta \psi^\alpha$. The integral Neumann boundary conditions can be viewed as imposing the Kelvin theorem on the boundary -- consider
\begin{equation}
    \frac \dd {\dd t}
    \int_{\p \domain}  \nabla (\psi^\alpha - \alpha \Delta \psi^\alpha) \cdot \normal = 0,
\end{equation}
and apply the divergence theorem.

In our FEM discretisation, we impose only Dirichlet boundary conditions.
% as can be seen from the definition of the approximation space $W^k_\delta(\domain)$. 
If the integral Neumann boundary conditions are not imposed, then for Proposition \ref{prop: TQG alpha conservation} to hold, we necessarily require $\psi^\alpha$ and $\Delta \psi^\alpha$ on $\p \domain$ to be \emph{zero}.
\end{remark}

We now analyse the conservation properties of our spatially discretised $\alpha$-TQG system. 
Let $\langle \cdot, \cdot \rangle_{H^1(\domain)}$ be the $H^1(\domain)$ inner product.
Define the numerical total energy
\begin{equation}\label{eq: numerical energy}
    E^\alpha_\delta(t) = 
    \frac12
    \langle \psi^\alpha_\delta
    , \tilde \psi_\delta
    \rangle_{H^1(\domain)}
    % L_1(\psi^\alpha_\delta, \tilde\psi_\delta)
    - 
    \frac12 
    \langle \rmh_\delta, b^\alpha_\delta \rangle_\domain,
\end{equation}
% \CHANGE{CHECK: If $\rmh_h \in W_h^k$ and $b_h \in V_h^k$, how is $\langle \rmh_h, b_h \rangle_\Omega$ defined? If $W_h^k \subset V_h^k$ then it's ok.}
in which $\psi_\delta^\alpha, \tilde{\psi}_\delta \in W_\delta^\alpha(\domain)$ and $b_\delta^\alpha\in V_\delta^k(\domain)$ are the numerical approximations of $\psi^\alpha$, $\tilde{\psi}$ and $b^\alpha$ respectively.
Define the numerical casimir functional
\begin{equation}\label{eq: TQG numerical casimirs}
C_{\delta}^\alpha(t; \Psi, \Phi ):= \langle\Psi(b_\delta^\alpha),1 \rangle_\domain
+ \langle \omega_\delta^\alpha \Phi(b_\delta^\alpha) \rangle_\domain, 
\quad \Psi, \Phi \in C^\infty.
\end{equation}

\begin{lemma} 
With boundary conditions \eqref{eq: tqg boundary conditions numerical}
\begin{equation}
    \frac \dd {\dd t} E^\alpha_\delta(t) = 0
\end{equation}
for $\alpha = 0$.
\end{lemma}
In other words, the semi-discrete discretisation conserves energy in the TQG case.
\begin{proof}
We consider $\dd/\dd_t$ evaluated at an arbitrary fixed value $t_0$.
First note that when $\alpha=0$, we have $\psi^\alpha_\delta = \tilde \psi_\delta$. Then, from \eqref{eq: psi bilinear form} we have
\begin{align}
    2E_\delta^\alpha(t) 
    % &=  L_1(\psi_\delta^\alpha, \tilde{\psi}_\delta) - \langle \rmh_\delta, b_\delta^\alpha \rangle_\Omega \nonumber \\
    &= L_1 (\psi_\delta^\alpha, {\psi}^\alpha_\delta) - \langle \rmh_\delta, b_\delta^\alpha \rangle_\Omega
    \label{eq: TQG total energy numerical}
\end{align}
% Differentiating the first term with respect to time, we get 
% \begin{equation}
% \frac \dd {\dd t}\Big|_{t=t_0} L_1(\psi^\alpha_\delta, \tilde{\psi}_\delta) = L_1(\p_t \psi^\alpha_\delta, \tilde{\psi}_\delta)\big|_{t=t_0}
% + L_1(\psi^\alpha_\delta, \p_t \tilde{\psi}_\delta)\big|_{t=t_0}.
% \end{equation}
For the first term in \eqref{eq: TQG total energy numerical}, following \eqref{eq: TQG psi eqn weak discretised} we have
\begin{align}
    % \left.\frac \dd {\dd t}\right|_{t=t_0} L_1(\tilde\psi_\delta, \phi_\delta) = 
    % \left.L_1(\p_t \tilde\psi_\delta, \phi_\delta)\right|_{t=t_0} 
    % &= \left.\frac \dd {\dd t}\right|_{t=t_0} F_{\omega^\alpha_\delta - f^\alpha_\delta}(\phi_\delta) = - \left.\langle\p_t \omega^\alpha_\delta, \phi_\delta \rangle_\domain \right|_{t=t_0} 
    % \nonumber \\
    \left.L_1(\p_t \psi_\delta, \phi_\delta)\right|_{t=t_0} = - \sum_{K\in \mathcal \domain_\delta} \left.\langle\p_t \omega^\alpha_\delta, \phi_\delta \rangle_K \right|_{t=t_0},
    \quad 
    \forall \phi_\delta \in W_\delta^k(\domain).
    % \nonumber
\end{align}
% in which the test function $\phi_\delta \in W_\delta^k(\domain)$ is arbitrary. 
 Thus, substituting in the discretised equation \eqref{eq: TQG omega eqn weak discretised numerical flux} for $\omega^\alpha$, we obtain
\begin{align}
    % - L_1(\left.\p_t \tilde\psi_\delta, \phi_\delta)\right|_{t=t_0}
    - L_1(\left.\p_t \psi_\delta, \phi_\delta)\right|_{t=t_0}
    % &= 
    % \sum_{K\in \mathcal T_\delta} 
    % \big[\langle \omega_\delta \nabla^\perp \psi_\delta, \nabla\phi_\delta\rangle _{K}
    % - \langle \hat f_1(\omega^+_\delta,\omega^-_\delta, \nabla^\perp \psi_\delta\cdot\hat{n}),\phi_\delta^-\rangle _{\partial K} \nonumber \\
    % & \qquad 
    % + \langle b_\delta \nabla^\perp(\frac12 \rmh_\delta-\psi_\delta),\nabla\phi_\delta\rangle _K 
    % \nonumber \\
    % &\qquad
    % -\langle \hat f_2(b^+, b^-, \nabla^\perp (\frac12 \rmh_\delta - \psi_\delta)\cdot \normal ), \phi_\delta^-\rangle_{\p K} \big]_{t=t_0}.
    % \\
    % \sum_{K\in \domain_\delta} \langle \p_t \omega^\alpha_\delta, \nu_\delta \rangle _{K} 
&= 
\sum_{K\in \domain_\delta} 
\left[
\big\{
\langle (\omega^\alpha_\delta - b^\alpha_\delta)\nabla^{\perp}\psi^\alpha_\delta,\nabla\phi_\delta\rangle _{K} - \frac12\langle \nabla \cdot (b^\alpha_\delta \nabla^\perp h_\delta), \phi_\delta \rangle _K
\right.
% \\
% &\qquad\quad
% -\langle \omega^\alpha_\delta \nabla^\perp \psi^\alpha_\delta \cdot\normal,
% \phi_\delta^-
% \rangle _{\partial K_\text{ext}}
\nonumber
\\
&\qquad -
\left.
\langle \hat{f}_{\omega^\alpha}((\omega^\alpha_\delta - b^\alpha_\delta)^{+}, (\omega^\alpha_\delta - b^\alpha_\delta)^{-}, \nabla^\perp \psi_\delta^\alpha \cdot \normal),
\phi_\delta^ -
\rangle _{\partial K}
\big\}
\right]_{t=t_0},
\label{eq: TQG kinetic energy time differential}
\end{align}
in which 
% \eqref{eq: TQG kinetic energy time differential}, 
we can choose $\phi_\delta=[\psi^\alpha_\delta]_{t=t_0}$. This choice is consistent with the discretisation space $V_\delta^k(\domain)$ for $\omega^\alpha$, since $W_\delta^k(\domain) \subset V_\delta^k(\domain)$.
% {\color{red} (Not true, need more regularity) We also have $L_1(\phi, \tilde\psi_\delta) = L_1((1-\alpha\Delta)\phi, \psi_\delta),$ $\phi,\psi_\delta, \tilde \psi_\delta \in W_\delta^k(\domain)$}. 
% Further, assuming $\p_t \psi_\delta \in W_\delta^k(\domain)$, we get ${\color{red} \left.L_1(\p_t \psi_\delta^\alpha, \tilde\psi_\delta)\right|_{t=t_0} = \left.L_1(\p_t \tilde \psi_\delta, \psi_\delta)\right|_{t=t_0}}$.

Similarly, for the second term in \eqref{eq: TQG total energy numerical}, using \eqref{eq: TQG b eqn weak discretised numerical flux} we obtain
\begin{equation}
    \left.\frac \dd {\dd t}\right\vert_{t=t_0} \langle b^\alpha_\delta, \nu_\delta \rangle_\domain
    % &= \sum_{K\in  \domain_\delta} \langle \p_t b^\alpha_\delta, \nu_\delta \rangle_K \big\vert_{t=t_0}
    % \nonumber \\
    = \sum_{K\in \domain_\delta} \left[ 
    \big\{
        \langle b^\alpha_\delta\nabla^{\perp} \psi^\alpha_\delta, \nabla \nu_\delta\rangle _{K}  -
        \langle \hat{f}_{b^\alpha}(b_\delta^{\alpha, +},b_\delta^{\alpha, -},\nabla^{\perp}\psi^\alpha_\delta \cdot \normal), \nu_\delta^{-}\rangle _{\partial K}
    \big\}
    \right]_{t=t_0},
    \label{eq: TQG potential energy time differential}
\end{equation}
where we can choose $\nu_\delta = \rmh_\delta$.

Putting together \eqref{eq: TQG total energy numerical}, \eqref{eq: TQG kinetic energy time differential} and \eqref{eq: TQG potential energy time differential}, and substituting in $\rmh_\delta$ and $[\psi^\alpha_\delta]_{t=t_0}$ for the arbitrary choices, we obtain
\begin{align}
    2 \frac \dd {\dd t}\Big|_{t=t_0} E^\alpha_\delta(t)
    &= 
    - \sum_{K\in \domain_\delta} 
    \left[
    2 \Big\{
    \langle (\omega^\alpha_\delta - b^\alpha_\delta)
    \underbrace{
    \nabla^{\perp}
    \psi^\alpha_\delta,\nabla
    \psi^\alpha_\delta
    }_{=0}
    \rangle _{K} - \frac12\langle \nabla \cdot (b^\alpha_\delta \nabla^\perp h_\delta), \psi^\alpha_\delta
    \rangle _K
    \right.
    % \right.
    \nonumber
    \\
    &\qquad 
    -
    % \left.
    \left.
    \langle \hat{f}_{\omega^\alpha}((\omega^\alpha_\delta - b^\alpha_\delta)^{+}, (\omega^\alpha_\delta - b^\alpha_\delta)^{-}, \nabla^\perp \psi_\delta^\alpha \cdot \normal),
    {\psi^\alpha_\delta}^-
    \rangle _{\partial K}
    \Big\}
    \right.
    % \right]_{t=t_0}
    \nonumber
    % \\
    % & \qquad {\color{red} + L_1(\p_t \psi_\delta^\alpha, \tilde\psi_\delta)}
    % \nonumber
    \\
    & 
    % -\sum_{K\in \domain_\delta} 
    +
    \left. 
    %\left[
    \Big\{
        \underbrace{
        \langle
        b^\alpha_\delta\nabla^{\perp} \psi^\alpha_\delta, \nabla \rmh_\delta\rangle _{K}  
        }_{=- \langle
        b^\alpha_\delta\nabla^{\perp}
        \rmh_\delta, \nabla \psi^\alpha_\delta\rangle _{K}  }
        -
        \langle \hat{f}_{b^\alpha}(b_\delta^{\alpha, +},b_\delta^{\alpha, -},\nabla^{\perp}\psi^\alpha_\delta \cdot \normal), \rmh_\delta^{-}\rangle _{\partial K}
    \Big\}
    \right]_{t=t_0}
\end{align}
% \begin{align}
%     2 \frac d {dt}\Big|_{t=t_0} E_\delta(t) &= \sum_{K\in \mathcal T_\delta} 
%     \Big[
%     2 \underbrace{\langle \omega_\delta \nabla^\perp \psi_\delta, \nabla\psi_\delta\rangle _{K}}_{=0}
%     -2  \langle \hat f_1(\omega^+_\delta,\omega^-_\delta, \nabla^\perp \psi_\delta\cdot\hat{n}),\psi_\delta^-\rangle _{\partial K}
%     \nonumber \\
%     & \qquad 
%     + 2 \langle b_\delta \nabla^\perp(\frac12 \rmh_\delta\underbrace{-\psi_\delta),\nabla\psi_\delta}_{\text{gives $0$}}\rangle _K 
%     \nonumber \\
%     &\qquad
%     -2 \langle \hat f_2(b^+, b^-, \nabla^\perp (\frac12 \rmh_\delta - \psi_\delta)\cdot \normal ), \psi_\delta^-\rangle_{\p K} \nonumber \\
%     & \qquad 
%     + \langle b_\delta\nabla^{\perp}\psi_\delta, \nabla \rmh_\delta\rangle _{K}  -
%     \langle \hat{f}(b_\delta^{+},b_\delta^{-},\nabla^{\perp}\psi_\delta \cdot \hat{n}), \rmh_\delta^{-}\rangle _{\partial K} \Big]_{t=t_0}
%     \\
%     &= \sum_{K\in \mathcal T_\delta} 
%     \Big[
%     \langle b_\delta \nabla^\perp\rmh_\delta,\nabla\psi_\delta\rangle _K 
%     + \underbrace{\langle b_\delta\nabla^{\perp}\psi_\delta, \nabla \rmh_\delta\rangle _{K}}
%     _{= - \langle b_\delta \nabla^\perp \rmh_\delta, \nabla \psi_\delta\rangle_K}
%     \nonumber \\
%     & \qquad 
%     - 2 \langle \hat f_1(\omega^+_\delta,\omega^-_\delta, \nabla^\perp \psi_\delta\cdot\hat{n}),\psi_\delta^-\rangle _{\partial K}
%     \nonumber \\
%     &\qquad
%     -2 \langle \hat f_2(b^+, b^-, \nabla^\perp (\frac12 \rmh_\delta - \psi_\delta)\cdot \normal ), \psi_\delta^-\rangle_{\p K} \nonumber \\
%     & \qquad 
%     - \langle \hat{f}(b_\delta^{+},b_\delta^{-},\nabla^{\perp}\psi_\delta \cdot \hat{n}), \rmh_\delta^{-}\rangle _{\partial K} \Big]_{t=t_0}
% \end{align}
% Hence
\begin{align}
    \frac \dd {\dd t} E^\alpha_\delta(t) &= \sum_{K\in \mathcal \domain_\delta} 
    \Big[
    - \langle \hat f_{\omega^\alpha}((\omega^\alpha_\delta-b^\alpha_\delta)^+,(\omega_\delta^\alpha - b^\alpha_\delta)^-, \nabla^\perp \psi^\alpha_\delta\cdot\normal),{\psi^\alpha_\delta}^-\rangle _{\partial K}
    \nonumber \\
    % &\qquad
    % -2 \langle \hat f_2(b^+_\delta, b^-_\delta, \nabla^\perp (\frac12 \rmh_\delta - \psi_\delta)\cdot \normal ), \psi_\delta^-\rangle_{\p K} \nonumber \\
    & \qquad 
    - \frac12
    \langle \hat{f}_{b^\alpha}({b^\alpha_\delta}^{+},{b^\alpha_\delta}^{-},\nabla^{\perp}\psi^\alpha_\delta \cdot \normal), \rmh_\delta^{-}\rangle _{\partial K} \Big]_{t=t_0}
    \label{eq: numerical energy temp}
\end{align}
Since $\psi_\delta$ and $\rmh_\delta$ are continuous across element boundaries, we have $\psi_\delta^+ = \psi_\delta^-$ and $\rmh_\delta^+ = \rmh_\delta^-$.
Thus, if the numerical fluxes $\hat f_{\omega^\alpha}$ and $\hat f_{b^\alpha}$ satisfy the conservative property \eqref{eq: nflux conservative}, the sum of flux terms is zero.
\end{proof}

\begin{remark}
In order for our semi-discrete discretisation to conserve numerical energy when $\alpha > 0$, more regularity is required for the approximation space for $\psi^\alpha_\delta$. Additionally, the current scheme coupled with the time stepping algorithm do not conserve  casimirs. For future work, we look to explore casimir conserving schemes for the model.
\end{remark}

% \begin{lemma}

% \end{lemma}


\subsubsection{Time stepping}
% For the time stepping scheme, we follow \cite{gottlieb2005high} and
% use a strong stability preserving Runge Kutta method of order 3 (SSPRK3)
% with the  Courant--Friedrich--Lewy (CFL) condition being $1/3.$
To discretise the time derivative, we use the strong stability preserving Runge-Kutta of order 3 (SSPRK3) scheme, see \cite{Hesthaven2008}.
Writing the finite element spatial discretisation formally as 
\begin{equation}
    \partial_{t}b^\alpha_\delta={\rm f}_\delta(b^\alpha_\delta)
\end{equation}
where ${\rm f}_\delta$ is the discretisation operator that follows from \eqref{eq: TQG b eqn weak discretised numerical flux}, and
\begin{equation}
     \partial_t \omega = {\rm g}_\delta (\omega, b)
\end{equation}
where ${\rm g}_\delta$ is the discretisation operator that follows from \eqref{eq: TQG omega eqn weak discretised numerical flux}.
Let $b^{\alpha, n}_\delta$ and $\omega^{\alpha,n}_\delta$ denote the approximation of $b^\alpha_\delta$ and $\omega^\alpha_\delta$ at time step $t_n$.
The SSPRK3
time discretisation is as follows 
\begin{subequations}
\begin{align}
    b^{(1)} & = b^{\alpha,n}_\delta + \Delta t \ {\rm f}_\delta (b^{\alpha,n}_\delta)\\
	\omega^{(1)} & =\omega^{\alpha,n}_\delta+\Delta t \  {\rm g}_\delta\left(\omega^{\alpha,n}_\delta, b^{\alpha,n}_\delta \right)\\
	b^{\left(2\right)} 
	&=\frac{3}{4}b^{\alpha,n}_\delta +\frac{1}{4}\left(b^{\left(1\right)}+\Delta t \ {\rm f}_\delta\left(b^{\left(1\right)}\right)\right)\\
	\omega^{\left(2\right)} 
	&= \frac{3}{4}\omega^{\alpha,n}_\delta
	+\frac{1}{4}\left(\omega^{\left(1\right)}+\Delta t \  {\rm g}_\delta\left(\omega^{\left(1\right)}, b^{(1)}\right)\right)\\
	b^{\alpha,n+1}_\delta & =\frac{1}{3}b^{\alpha,n}_\delta+\frac{2}{3}\left(b^{\left(2\right)}+\Delta t \  {\rm f}_\delta\left(b^{\left(2\right)}\right)\right)\\
	\omega^{\alpha,n+1}_\delta & =\frac{1}{3}\omega^{\alpha,n}_\delta
	+\frac{2}{3}\left(\omega^{\left(2\right)}+\Delta t \  {\rm g}_\delta\left(\omega^{\left(2\right)}, b^{(2)}\right)\right)
\end{align}
\end{subequations}
where $\Delta t = t_{n+1}-t_{n}$ each $n$. 

% \begin{align*}
%     b^{(1)} & = b^n + \Delta f_\delta (b^n)
%     \\
% 	\omega^{(1)} & =\omega^{n}+\Delta g_\delta\left(\omega^{n}, b^n\right)
% 	\\
% 	b^{\left(2\right)} 
% 	&=\frac{3}{4}b^{n}+\frac{1}{4}\left(b^{\left(1\right)}+\Delta f_\delta\left(b^{\left(1\right)}\right)\right)
% 	\\
% 	& = \frac{3}{4}b^{n}+
% 	\frac{1}{4}b^n + \frac{1}{4}\Delta f_h (b^n)+
% 	\frac{1}{4}\Delta 
% 	f_\delta\left(b^n + \Delta f_h (b^n)\right)
% 	\\
% 	&= b^{n}+
% 	\frac{1}{4}\Delta f_h (b^n)+
% 	\frac{1}{4}\Delta 
% 	f_\delta(b^{(1)})
% 	\\
% 	\omega^{\left(2\right)} & =\frac{3}{4}\omega^{n}+\frac{1}{4}\left(\omega^{\left(1\right)}+\Delta g_\delta\left(\omega^{\left(1\right)}, b^{(1)}\right)\right)
% 	\\
% 	& =
% 	\frac{3}{4}\omega^{n}+\frac{1}{4}\Big[\omega^{n}+\Delta g_\delta\left(\omega^{n}, b^n\right)+\Delta g_\delta\big(
% 	\omega^{(1)},
% 	b^{(1)}\big)\Big]
% 	\\
% 	& =
% 	\omega^{n} + \frac14\Big[\Delta g_\delta\left(\omega^{n}, b^n\right)+\Delta g_\delta\big(
% 	\omega^{(1)},
% 	b^{(1)}\big)\Big]
% % 	\\
% % 	& =
% % 	\omega^{n} + \frac14\Big[
% % 	2\Delta g_\delta\left(\omega^{n}, b^n\right)
% % 	+ \Delta^2 g(\omega^n, b^n) g_h_x(\omega^n , b^n)
% % 	+ \Delta^2 f_h(b^n) g_h_y(\omega^n, b^n) +O(\Delta^3)
% % 	]
% 	\\
% 	& = 
% 	\omega^{n} + \frac12
% 	\Delta g_\delta\left(\omega^{n}, b^n\right)
% 	+ O(\Delta^2)
% 	\\
% 	b^{n+1} & =\frac{1}{3}b^{n}+\frac{2}{3}
% 	\left(b^{\left(2\right)}
% 	+\Delta f_\delta\left(b^{\left(2\right)}\right)\right)
% 	\\
% 	&=b^{n}
% 	+ 
% 	\left(
% 	\frac16\Delta f_h (b^n)+
% 	\frac16\Delta 
% 	f_\delta(b^{(1)})
% 	+
% 	\frac23\Delta f_\delta
% 	\left(
% 	b^{\left(2\right)}
% 	\right)\right)
% 	\\
% 	&=
% 	b^{n}
% 	+ 
% 	\left(
% 	\frac13\Delta f_h (b^n)
% 	+ \frac16\Delta^2 f_h'(b^n) f_h(b^n) + O(\Delta^3)
% 	\right.\\
% 	&
% 	\left.
% 	+
% 	\frac23\Delta f_\delta
% 	(
% 	b^{n}+
% 	\frac{1}{4}\Delta f_h (b^n)+
% 	\frac{1}{4}\Delta 
% 	f_\delta(b^{(1)})
% 	)
% 	\right)
% 	\\
% 	&= b^n + \Delta f_h(b^n) + O(\Delta^2)
% 	\\
% 	\omega^{n+1} & =\frac{1}{3}\omega^{n}+\frac{2}{3}\left(\omega^{\left(2\right)}+\Delta g_\delta\left(\omega^{\left(2\right)}, b^{(2)}\right)\right)
% 	\\
% 	& =
% 	\frac{1}{3}\omega^{n}
% 	+
% 	\frac{2}{3}
% 	\left(
% 	\omega^{n} + \frac12
% 	\Delta g_\delta\left(\omega^{n}, b^n\right)
% 	+ O(\Delta^2)\right.
% 	\\
% 	& + \left. \Delta g_\delta
% 	\left(\omega^{n} + \frac12
% 	\Delta g_\delta\left(\omega^{n}, b^n\right)
% 	+ O(\Delta^2), b^{n}+
% 	\frac{1}{4}\Delta f_h (b^n)+
% 	\frac{1}{4}\Delta 
% 	f_\delta(b^{(1)})\right)\right)
% 	\\
% 	& =
% 	\omega^{n}
% 	+
% 	\frac{2}{3}
% 	\left(
% 	\frac12
% 	\Delta g_\delta\left(\omega^{n}, b^n\right)
% 	 + \Delta 
% 	g_\delta(\omega^n, b^n)+ O(\Delta^2)
% 	\right)
% 	\\
% 	& = \omega^n + \Delta g_h(\omega^n, b^n) + O(\Delta^2)
% \end{align*}

% In variational form, we have

% \begin{align}\left\langle v_\delta,\omega^{(1)}\right\rangle _{K} 
% & =\left\langle v_\delta,\omega^{n}\right\rangle _{K}
% -\Delta t
% \left(
% \left\langle \nabla v_\delta,-(\omega^{n}-b^n)\nabla^{\perp}\psi_\delta^{n}\right\rangle _{K}+\left\langle v_\delta,\omega^{n}\nabla^{\perp}\psi_\delta^{n}\cdot\hat{n}\right\rangle _{\partial K}
% \right)
% \nonumber
% \\
% & - \Delta t 
% \left(  
% \left\langle \nabla v_\delta,-b^{n}\nabla^{\perp}\rmh_\delta^{n}\right\rangle _{K}+\left\langle v_\delta,b^{n}\nabla^{\perp}\rmh_\delta^{n}\cdot\hat{n}\right\rangle _{\partial K}
% \right)
% \\
% \dots &
% % \left\langle v_\delta,\omega^{\left(2\right)}\right\rangle _{K} & =\frac{3}{4}\left\langle v_\delta,\omega^{n}\right\rangle _{K}+\frac{1}{4}\left\langle v_\delta,\omega^{\left(1\right)}\right\rangle _{K}\\
% % & \qquad-\frac{\Delta t}{4}\left(\left\langle \nabla v_\delta,-\omega^{\left(1\right)}\nabla^{\perp}\psi_\delta^{\left(1\right)}\right\rangle _{K}+\left\langle v_\delta,\omega^{\left(1\right)}\nabla^{\perp}\psi_\delta^{\left(1\right)}\cdot\hat{n}\right\rangle _{\partial K}\right)\\
% % \left\langle v_\delta,\omega^{n+1}\right\rangle _{K} & =\frac{1}{3}\left\langle v_\delta,\omega^{n}\right\rangle _{K}+\frac{2}{3}\left\langle v_\delta,\omega^{\left(2\right)}\right\rangle _{K}\\
% % & \qquad-\frac{2\Delta t}{3}\left(\left\langle -\omega^{\left(2\right)}\nabla^{\perp}\psi_\delta^{\left(2\right)},\nabla v_\delta\right\rangle _{K}+\left\langle v_\delta,\omega^{\left(2\right)}\nabla^{\perp}\psi_\delta^{\left(2\right)}\cdot\hat{n}\right\rangle _{\partial K}\right)
% \end{align}
% for each $K\in\mathcal{T}_\delta.$ 


\subsection{$\alpha$-TQG linear thermal Rossby wave stability analysis}\label{sec: numerics linear stability analysis}

% The regularised TQG model is
% \begin{align}
% \p_{t}b+\nabla\cdot(b\tilde{\bu}) & =0\\
% \p_{t}\omega+\nabla\cdot(\omega\tilde{\bu}) & =\nabla\cdot\left(b\tilde{\bu}-\frac{1}{2}b\nabla^{\perp}\rmh\right)\\
% \tilde{\bu} & =\nabla^{\perp}\tilde{\psi}\\
% \bu & =\nabla^{\perp}\psi\\
% \omega & =(\Delta-1)\psi+f.\\
% \psi & =(1-\alpha^{2}\Delta)\tilde{\psi}
% \end{align}

A dispersion relation for the TQG system was derived in \cite{Holm2021}. There, the authors showed that the linear thermal Rossby waves of the TQG system possess high wavenumber instabilities. More specifically, the Doppler-shifted phase speed of these waves becomes complex at sufficiently high wavenumbers. However, the growth rate of the instability decreases to zero as $|\bk|^{-1}$, in the limit that $|\bk|\to\infty$. Consequently, the TQG dynamics is linearly well-posed in the sense of Hadamard. That is, the TQG solution depends continuously on initial conditions. 
In this subsection, using the same equilibrium state as in \cite{Holm2021}, we derive a dispersion relation for the  thermal Rossby wave solutions of the linearised $\alpha$-TQG system. Again the Doppler-shifted phase speed of these waves becomes complex at sufficiently high wavenumbers. However, in this case, the growth rate of the instability decreases to zero as $|\bk|^{-2}$, in the limit that $|\bk|\to\infty$. In the limit that $\alpha$ tends to zero, one recovers the TQG dispersion relation derived in \cite{Holm2021}.

For the reader's convenience, we repeat the equations solved by the pair of variables $(b^\alpha,\omega^\alpha)$ in the $\alpha$-TQG system in \eqref{ceAlpha}--\eqref{meAlpha}, as formulated now in vorticity-streamfunction form with fluid velocity given by ${\bu}^\alpha =\nabla^\perp \psi^\alpha$. This formulation is given by
\begin{align}
\frac{\partial}{\partial t} b^\alpha + J(\psi^\alpha,b^\alpha) &= 0,
\label{ceZero-redux}\\
\frac{\partial}{\partial t}\omega^\alpha + J(\psi^\alpha,\omega^\alpha-b^\alpha) &= -\frac{1}{2}J(h,b^\alpha),
\label{meZero-redux}\\
\omega^\alpha &= (\Delta-1) (1-\alpha \Delta )\psi^\alpha + f.
\label{constrtZero-redux}
\end{align}
Here, as before, $J(a,b)=\nabla^\perp a\cdot \nabla b=a_x b_y - b_x a_y$ denotes the Jacobian of any smooth functions $a$ and $b$ defined on the $(x,y)$ plane.


Equilibrium states of the $\alpha$-TQG system in the equations \eqref{ceZero-redux}-\eqref{constrtZero-redux} satisfy $J(\psi^\alpha_e, \omega^\alpha_e) = J(\psi^\alpha_e, b^\alpha_e)=J(h, b^\alpha_e)=0.$
The equilibrium TQG state considered in \cite{Holm2021} was given via the specification of the following
gradient fields 
\[
\begin{array}{c}
\nabla\psi^\alpha_{e}=-U\yhat,\ \nabla\omega^\alpha_{e}=(U-\beta)\yhat,\ \nabla f=-\beta\yhat\\
\\
\nabla b^\alpha_{e}=-B\yhat,\ \nabla\rmh=-H\yhat
\end{array}
\]
where we have taken $f=1-\beta y$ and the equilibrium parameters $U, \beta, B, H \in \reals$ are all constants.
% For the $\alpha$-TQG equations, we have the following specification for the $\alpha$-regularised stream function corresponding to the equilibrium state
% \[
% \nabla{\psi}^\alpha_{e}=-U\yhat.
% \]
% which follows from a particular solution to
% \[
% (1-\alpha^{2}\Delta)\nabla\tilde{\psi}_{e}=\nabla\psi_{e}.
% \]
Linearising the $\alpha$-TQG system around the steady state produces the
following evolution equations for the perturbations $\omega'$, $b'$
and ${\psi}'$
\begin{subequations}\label{eq: linear alpha tqg}
\begin{align}
\omega_{t}'+U\omega'_{x}+(U+B-\beta){\psi}_{x}' & =(U-H/2)b'_{x}
\\
b'_{t}+Ub_{x}'-B{\psi}_{x}' & =0\\
{\color{blue}\Big((1-\alpha\Delta)(1-\Delta)\Big)}{\psi}' & =-\,\omega'. \label{eq: linear alpha tqg psi}
\end{align}
\end{subequations}
Since these equations are linear with constant coefficients, one has
the plane wave solutions
\[
\omega'=e^{i(\bk\cdot\bx-\nu t)}\hat{\omega},\quad b'=e^{i(\bk\cdot\bx-\nu t)}\hat{b},\quad{\psi}'=e^{i(\bk\cdot\bx-\nu t)}\hat{{\psi}}.
\]
Further, from \eqref{eq: linear alpha tqg psi} we obtain
\[
-\,\hat{\omega}={\color{blue}(|\bk|^{2}+1)(\alpha|\bk|^{2}+1)}\hat{{\psi}}.
\]
Substituting these solutions into the linearised equations we have
\[
\begin{aligned}(\nu-kU)\hat{\omega}-k(U+B-\beta)\hat{{\psi}} & =-k(U-H/2)\hat{b}\\
\left(\nu-kU\right)\hat{b} & =-kB\hat{{\psi}}
\end{aligned}
\]
where $k$ is the first component of $\bk$.
From the above we obtain a quadratic formula for the Doppler-shifted phase speed $C = C(\alpha):=\left(\nu(\alpha)-kU\right)/k$
\[
C^{2}(|\bk|^{2}+1)(\alpha|\bk|^{2}+1)+CX+Y=0.
\]
where $X:=U+B-\beta$
and $Y:=(U-H/2)B$. Thus, the dispersion relation for the thermal Rossby wave for TQG possesses two branches, 
corresponding to two different phase velocities,
\begin{equation}\label{eq: doppler shift phase speed}
C(\alpha)=\frac{-X\pm\sqrt{X^{2}-4Y{\color{blue}(|\bk|^{2}+1)(\alpha|\bk|^{2}+1)}}}
{2{\color{blue}(|\bk|^{2}+1)(\alpha|\bk|^{2}+1)}}.
\end{equation}
% \[
% \begin{aligned}C(\alpha) & =\frac{-X\pm\sqrt{X^{2}-4Y\left(\alpha|\bk|^{4}+(1+\alpha)|\bk|^{2}+1\right)}}{2\left(\alpha|\bk|^{4}+(1+\alpha)|\bk|^{2}+1\right)}\\
%  & =-\frac{X}{2\left(\alpha|\bk|^{4}+(1+\alpha)|\bk|^{2}+1\right)}\\
%  & \qquad\pm\frac{\sqrt{X^{2}-4Y\left(\alpha|\bk|^{4}+(1+\alpha)|\bk|^{2}+1\right)}}{2\left(\alpha|\bk|^{4}+(1+\alpha)|\bk|^{2}+1\right)}\\
%  & =-\frac{X}{2\left(\alpha|\bk|^{4}+(1+\alpha)|\bk|^{2}+1\right)}\\
%  & \qquad\pm\frac{1}{2}\sqrt{\frac{1}{\left(\alpha|\bk|^{4}+(1+\alpha)|\bk|^{2}+1\right)}\left(\frac{X^{2}}{\left(\alpha|\bk|^{4}+(1+\alpha)|\bk|^{2}+1\right)}-4Y\right)}
% \end{aligned}
% \]
Upon setting $\alpha=0$ in \eqref{eq: doppler shift phase speed}, we recover the Doppler-shifted phase speed of {\color{blue}thermal Rossby waves for the TQG system in \cite{Holm2021}. When $\alpha=0$, $B=0$, and $U=0$ in \eqref{eq: doppler shift phase speed}, we recover the standard dispersion relation for QG Rossby waves in non-dimensional variables.} 

As discussed in \cite{Holm2021} for the TQG system, when $Y>0$, {\color{blue}the Doppler shifted phase velocity in \eqref{eq: doppler shift phase speed} for the linearised wave motion becomes complex at high wavenumber $|\bk| \gg 1$; namely for $(|\bk|^{2}+1)(\alpha|\bk|^{2}+1)\ge X^{2}/(4Y)$, for both branches of the dispersion relation. However, the growth-rate of the instability found from the imaginary part of $C(\alpha)$ in \eqref{eq: doppler shift phase speed} decays to zero as $O( |\bk|^{-2})$, for $|\bk|\gg1$. Indeed, the linear stability analysis leading to $C(\alpha)$ predicts that the maximum growth rate occurs at a finite wavenumber $|\bk|_{\max}$ which depends on the value of $\alpha$, beyond which the growth rate of the linearised TQG wave amplitude falls rapidly to zero. One would expect that simulated solutions of $\alpha$-TQG would be most active at the length-scale corresponding to $|\bk|_{\max}$, at which the linearised thermal Rossby waves are the most unstable}. If this maximum activity length-scale is near the grid truncation size, then numerical truncation errors could cause additional numerical stability issues! We have experience such problems during our testing of the numerical algorithm for the TQG system. Even for equilibrium solution ``sanity" check tests, we have found that unless the time step was taken to be incredibly small, high wavenumber truncation errors have caused our numerical solutions to eventually blow up.

\begin{figure}[h!]
\centering
\includegraphics[width=0.6\textwidth]{Kato Existence/growth_rate.png}
\caption{An example of the growth-rate of {\color{blue}linearised TQG waves as determined from the imaginary part of $C(\alpha)$ in equation \eqref{eq: doppler shift phase speed}}, plotted for different values of $\alpha$. We observe that increasing $\alpha$ shifts the wavenumber at the maximum growth-rate to lower values.}
\label{fig: growth rate}
\end{figure}

The magnitude of $\alpha$ {\color{blue} controls the unstable growth rate of linearised TQG waves at asymptotically high wavenumbers. That is, the presence of $\alpha$} regularises the wave activity at high wavenumbers, see Figure \ref{fig: growth rate}. Thus, from the perspective of numerics, the $\alpha$ regularisation is available to control numerical problems that may arise from the inherent model instability {\color{blue}at high wavenumbers}, without the need for additional dissipation terms in the equation.

\subsection{Numerical example}\label{sec: numerics example}
The numerical setup we consider for this paper is as follows.
The spatial domain $\domain$ is an unit square with doubly periodic boundaries.
We chose to discretise $\domain$ using a grid that 
consists of $256\times256$ cells, i.e. $\cardinality(\domain_\delta) = 256\times256$. This was the maximum resolution we could computationally afford, to obtain results over a reasonable amount of time.

We computed $\alpha$-TQG solutions for the following values of $\alpha$ -- $\frac{1}{16^{2}},\frac{1}{32^{2}},\frac{1}{64^{2}},\frac{1}{128^{2}},\frac{1}{180^{2}},\frac{1}{220^{2}},\frac{1}{256^{2}}$ and $0$.
Note when $\alpha=0$ we get the TQG system.
For all cases, the following initial conditions were used,
% \begin{subequations}
% \begin{equation}
% \begin{equations}
\begin{align}
\omega(0,x,y) & =\sin(8\pi x)\sin(8\pi y)+0.4\cos(6\pi x)\cos(6\pi y)\label{eq: pv initial condition}\\
 & \quad+0.3\cos(10\pi x)\cos(4\pi y)+0.02\sin(2\pi y)+0.02\sin(2\pi x) \nonumber \\
b(0,x,y) & =\sin(2\pi y)-1, \label{eq: buoyancy initial condition}
\end{align}
% \end{equation}
% \end{subequations}
% \end{equations}
see Figure \ref{fig: initial conditions} for illustrations,
as well as the following bathymetry and rotation fields
% \begin{equations}
\begin{align}
h(x,y) & =\cos(2\pi x)+0.5\cos(4\pi x)+\frac{1}{2}\cos(6\pi x) \label{eq: bathymetry}\\
f(x,y) & =0.4\cos(4\pi x)\cos(4\pi y). \label{eq: rotation}
\end{align}
% \end{equations}
For time stepping, we used $\Delta t = 0.0005$ in all cases to facilitate comparisons. This choice satisfies the CFL condition for the $\alpha=0$ case. 

We computed each solution for $5000$ time steps. See \cite{youtube_2021} for a video of the full simulation. Figures \ref{fig: snapshot buoyancy}, \ref{fig: snapshot pv} and \ref{fig: snapshot velocity magnitude} show $\alpha$-TQG solution snapshots of buoyancy, potential vorticity and velocity magnitude respectively, at the $1280$'th and $2600$'th time steps, for $\alpha$ values $0, \frac1{128^2}, \frac1{64^2}$ and $\frac1{16^2}$. The interpretation of the regularisation parameter $\alpha$ is that its square root value corresponds to the fraction of the domain's length scale that get regularised.
At the $1280$'th time step, the flows are in early spin-up phase.
At the $2600$'th time step, although the flows are still in spin-up phase, much more flow features have developed.
The sub-figures illustrate via comparisons, how $\alpha$ controls the development of small scale features and instabilities. Increasing $\alpha$ leads to more regularisation at larger scales.

In view of Proposition \ref{prop:alphaConv}, we investigated numerically the convergence of $\alpha$-TQG to TQG using our numerical setup. Consider the relative error between TQG buoyancy and $\alpha$-TQG buoyancy, 
\begin{align}
e_b(t, \alpha) &:= \frac{\|b(t) - b^\alpha(t)\|_{H^1}}{\|b(t)\|_{H^1}}\label{eq: relative error buoyancy}
\end{align}
and the relative error between TQG potential vorticity and $\alpha$-TQG potential vorticity,
% \begin{subequations}
\begin{align}
    e_\omega(t, \alpha) &:= \frac{\|\omega(t) - \omega^\alpha(t)\|_{L^2}}{\|\omega(t)\|_{L^2}}.\label{eq: relative error pv}
\end{align}
% \end{subequations}
% \end{equation}
The norms were chosen in view of Proposition \ref{prop:alphaConv}.
Figures \ref{fig: relative error buoyancy time series} and \ref{fig: relative error pv time series} show plots of $e_b(t, \alpha)$ and $e_\omega(t, \alpha)$
as functions of time only, for fixed $\alpha$ values $\frac{1}{16^2}, \frac{1}{32^2}, \frac1{64^2}, \frac1{128^2}$ and $\frac1{220^2}$, from the initial time up to and including the $2800$'th time step.
We observe that starting from $0$, the relative errors $e_b$ and $e_\omega$ initially increase over time but plateau at around and beyond the $2000$'th time step. 
Up to the $1400$'th time step, 
the plotted relative errors remain less than $1.0$, and are arranged in the ascending order of $\alpha$, i.e. smaller $\alpha$'s give smaller relative errors.

We note that, if we compare and contrast the relative error results with the solution snapshots of buoyancy and potential vorticity, particularly at the $2600$'th time step (shown in Figures \ref{fig: snapshot buoyancy 1.30} and \ref{fig: snapshot pv 1.30}), we observe "discrepancies" -- for lack of a better term -- between the results. For example, in Figure \ref{fig: snapshot buoyancy 1.30}, if we compare the $\alpha=\frac1{128^2}$ snapshot with the $\alpha=\frac1{16^2}$ one, the former
show small scale features that are much closer to those that exist in the reference TQG $\alpha=0$ solution. However, according to the relative error measurements, 
% especially $e_b$, 
the two regularised solutions are more or less equivalent in their differences to the reference TQG solution at time step $2600$.

If we fix the value of the time parameter in $e_b(t,\alpha)$ and $e_\omega(t, \alpha)$, and vary $\alpha$, we can estimate the convergence rate of $\alpha$-TQG to TQG for our numerical setup. Proposition \ref{prop:alphaConv} predicts a convergence rate of $1$ in $\alpha$, using the $H^1$ norm on the buoyancy differences and the $L^2$ norm on the potential vorticity differences.
Note that, in \eqref{rateOfConv}, the left hand side evaluates a supremum over a given compact time interval. We see in Figures \ref{fig: relative error buoyancy time series} and \ref{fig: relative error pv time series} that the relative errors are monotonic up to around the $1500$'th time step mark. So for a given time point $T$ between the initial time and the $1500$'th time step, we assume we can evaluate $e_b$ and $e_\omega$ at $T$ to estimate the supremum over $[0,T]$. 

Figures \ref{fig: relative error convergence buoyancy} and \ref{fig: relative error convergence pv} show plots -- in log-log scale -- of $e_b$ and $e_\omega$ as functions of $\alpha$ only at the $600$'th, $800$'th, $1000$'th and $1200$'th time steps, for all the chosen $\alpha$ values. These numbers of time steps correspond to $T=0.3$, $T=0.4$, $T=0.5$ and $T=0.6$ respectively. We also plotted in Figures \ref{fig: relative error convergence buoyancy} and \ref{fig: relative error convergence pv} linear functions of $\alpha$ to provide reference order 1 slopes.
Comparing the results to the reference, we see that the theoretical convergence rate of 1 is attained for $T=0.3$ ($600$'th time step), $T=0.4$ ($800$'th time step) and $T=0.5$ ($1000$'th time step). However for $T=0.6$ ($1200$'th time step), the convergence rates are at best order $1/2$.


% initial condition plot
\begin{figure}
\centering
\includegraphics[width=0.6\textwidth]{Kato Existence/initial_conditions_buoyancy_pv.png}
\caption{Initial conditions -- buoyancy \eqref{eq: buoyancy initial condition} on the left, and potential vorticity \eqref{eq: pv initial condition} on the right. The different colours of the PV plot correspond to positive and negative values of PV, which can be interpreted as clockwise and anticlockwise eddies respectively.}
\label{fig: initial conditions} 
\end{figure}

% show figures of solution snapshots
\begin{figure}[t]
\centering
 \begin{subfigure}[b]{0.6\textwidth}
     \centering
     \includegraphics[trim={340 25 196 5},clip,width=\textwidth]{Kato Existence/alpha_convergence_bouyancy_comparisons_t_0.64.png}
     \caption{}
     \label{fig: snapshot buoyancy 0.64}
 \end{subfigure}
 \vfill
 \begin{subfigure}[b]{0.6\textwidth}
     \centering
     \includegraphics[trim={340 25 196 5},clip, width=\textwidth]{Kato Existence/alpha_convergence_bouyancy_comparisons_t_1.30.png}
     \caption{}
     \label{fig: snapshot buoyancy 1.30}
 \end{subfigure}
 \caption{Comparisons of solution snapshots of the $\alpha$-TQG buoyancy field that correspond to four different values of $\alpha$, at two different points in time. Potential vorticity and velocity magnitude snapshots of the same solutions are shown in Figure \ref{fig: snapshot pv} and Figure \ref{fig: snapshot velocity magnitude} respectively. Shown in each sub-figure are the results corresponding to $\alpha = 0$ (top left), $\alpha = \frac1{128^2}$ (top right), $\alpha = \frac1{64^2}$ (bottom right) and $\alpha = \frac1{16^2}$ (bottom left). When $\alpha=0$, the solution is of the TQG system. Sub-figure (A) shows the solutions at the $1280$'th time step, or equivalently when $t=0.64$. Sub-figure (B) shows the solutions at the $2600$'th time step, or equivalently when $t=1.30$. The flows in both sub-figures are at different stages of spin-up, with the flow at $t=1.30$ showing more developed features. The $\alpha$ parameter is  interpreted as the fraction of the domain's length-scale squared value at which regularisation is applied. Due to regularisation, the flows do develop differently. Nevertheless, we observe that as $\alpha$ gets smaller, the $\alpha$-TQG flow features converge to that of the TQG flow.}
 \label{fig: snapshot buoyancy}
\end{figure}

\begin{figure}[t]
\centering
 \begin{subfigure}[b]{0.6\textwidth}
     \centering
     \includegraphics[trim={340 25 196 5},clip,width=\textwidth]{Kato Existence/alpha_convergence_pv_comparisons_t_0.64.png}
     \caption{}
     \label{fig: snapshot pv 0.64}
 \end{subfigure}
 \vfill
 \begin{subfigure}[b]{0.6\textwidth}
     \centering
     \includegraphics[trim={340 25 196 5},clip, width=\textwidth]{Kato Existence/alpha_convergence_pv_comparisons_t_1.30.png}
     \caption{}
     \label{fig: snapshot pv 1.30}
 \end{subfigure}
 \caption{Comparisons of solution snapshots of the $\alpha$-TQG potential vorticity field that correspond to four different values of $\alpha$, at two different points in time. See the caption of Figure \ref{fig: snapshot buoyancy} for explanations of the arrangements of these plots. Buoyancy and velocity magnitude snapshots of the same solutions are shown in Figure \ref{fig: snapshot buoyancy} and Figure \ref{fig: snapshot velocity magnitude} respectively. As in Figure \ref{fig: initial conditions}, the different colours of the PV field correspond to positive and negative values of PV, which can be interpreted as clockwise and anticlockwise eddies respectively. In sub-figure (B), we observe more clearly the regularisation effects of $\alpha$. As $\alpha$ 
 increases, the flows develop in different ways -- features at smaller scales no longer develop, and larger features evolve differently as a result.
 Nevertheless, we observe that as $\alpha$ gets smaller, the $\alpha$-TQG flow features converge to that of the TQG flow.}
 \label{fig: snapshot pv}
\end{figure}

\begin{figure}[t]
\centering
 \begin{subfigure}[b]{0.6\textwidth}
     \centering
     \includegraphics[trim={340 25 151 5},clip,width=\textwidth]{Kato Existence/alpha_convergence_velocity_comparisons_t_0.64.png}
     \caption{}
     \label{fig: snapshot velocity magnitude 0.64}
 \end{subfigure}
 \vfill
 \begin{subfigure}[b]{0.6\textwidth}
     \centering
     \includegraphics[trim={340 25 151 5},clip, width=\textwidth]{Kato Existence/alpha_convergence_velocity_comparisons_t_1.30.png}
     \caption{}
     \label{fig: snapshot velocity magnitude 1.30}
 \end{subfigure}
 \caption{Comparisons of solution snapshots of the $\alpha$-TQG velocity magnitudes that correspond to four different values of $\alpha$, at two different points in time. See the caption of Figure \ref{fig: snapshot buoyancy} for explanations of the arrangements of these plots. 
 Buoyancy and potential vorticity snapshots of the same solutions are shown in Figure \ref{fig: snapshot buoyancy} and Figure \ref{fig: snapshot pv} respectively. 
%  Here we used the Turbo colour scheme to better distinguish the different ranges of values. 
 Using the same scale for colouring, we observe in both sub-figures the strength of the colours weaken as $\alpha$ increases. This indicates smoothing of large velocity magnitudes.
 Additionally, in sub-figure (B), we observe how features at smaller scales get smoothed out. In particular, in the $\alpha=\frac1{16^2}$ plot, we see that essentially only large scale vorticies remain. Hence, considering the velocity field as a part of the system's nonlinear advection operator, these figures help us to better visualise how the flow features developed in Figure \ref{fig: snapshot buoyancy} and Figure \ref{fig: snapshot pv}. }
%  We observe that as $\alpha$ gets smaller, the $\alpha$-TQG flow features converge to that of the TQG flow. }
 \label{fig: snapshot velocity magnitude}
\end{figure}

% show figures of error convergence
\begin{figure}[t]
\centering
 \begin{subfigure}[b]{0.7\textwidth}
     \centering
     \includegraphics[width=\textwidth]{Kato Existence/relative_error_buoyancy.png}
     \caption{
    %  Plots of the bouyancy relative error function $e_b(t, \alpha)$ defined in \eqref{eq: relative error buoyancy} as a function of time only for different values of $\alpha$.
     }
     \label{fig: relative error buoyancy time series}
 \end{subfigure}
%  \hfill
 \begin{subfigure}[b]{0.7\textwidth}
     \centering
     \includegraphics[width=\textwidth]{Kato Existence/relative_error_pv.png}
     \caption{
    %  Plots of the potential vorticity relative error function $e_\omega(t, \alpha)$ defined in \eqref{eq: relative error pv} as a function of time for different values of $\alpha$.
     }
     \label{fig: relative error pv time series}
 \end{subfigure}
 \caption{Sub-figures (A) and (B) show, respectively, plots of the relative error functions $e_b(t, \alpha)$ and $e_\omega(t, \alpha)$
 as functions of time only, for the fixed $\alpha$ values $\frac{1}{16^2}$, $\frac1{32^2}$, $\frac1{64^2}$, $\frac1{128^2}$ and $\frac1{220^2}$. See equations \eqref{eq: relative error buoyancy} and \eqref{eq: relative error pv} for the definitions of $e_b$ and $e_\omega$ respectively. The plots are shown from $t=0$ up to and including $t=1.4$, which is equivalent to $2800$ time steps using $\Delta t = 0.0005$.
 We observe that, starting from $0$, all plots of  $e_b$ and $e_\omega$ increase initially, and plateau at around the $2000$'th time step. Further, up to the $1400$'th time step the plotted relative errors remain less than $1.0$ and are arranged in the ascending order of $\alpha$. Relating these relative error results at the $2600$'th time step to the solution snapshots at the same time point (shown in figures \ref{fig: snapshot buoyancy 1.30} and \ref{fig: snapshot pv 1.30}), we see that although the snapshots show convergence of flow features, the relative error values suggest all the $\alpha$-TQG solutions are more or less equally far away from the TQG flow.
 }
  \label{fig: relative errors time series}
\end{figure}

\begin{figure}[t]
\centering
 \begin{subfigure}[b]{0.7\textwidth}
     \centering
     \includegraphics[width=\textwidth]{Kato Existence/relative_error_convergency_buoyancy.png}
     \caption{}
     \label{fig: relative error convergence buoyancy}
 \end{subfigure}
%  \hfill
 \begin{subfigure}[b]{0.7\textwidth}
     \centering
     \includegraphics[width=\textwidth]{Kato Existence/relative_error_convergency_pv.png}
     \caption{}
     \label{fig: relative error convergence pv}
 \end{subfigure}
 \caption{
 Sub-figures (A) and (B) show, respectively, plots in log-log scale of the relative error functions $e_b(t, \alpha)$, and $e_\omega(t, \alpha)$
 as functions of $\alpha$ only, at the fixed time values $t=0.3$ (equivalently at the $600$'th time step), $t=0.4$ (equivalently at the $800$'th time step), $t=0.5$ (equivalently at the $1000$'th time step) and $t=0.6$ (equivalently at the $1200$'th time step). 
  In view of Proposition \ref{prop:alphaConv}, we assumed that, based on the initial monotonicity of the relative errors (see Figure \ref{fig: relative errors time series}), the supremum over $[0,T]$ in \eqref{rateOfConv} can be estimated by evaluating $e_b$ and $e_\omega$ at $T$.
 Proposition \ref{prop:alphaConv} predicts that up to a certain time, the rate of convergence of $e_b$ and $e_\omega$ to $0$ should be no less than order 1 in $\alpha$.
 In both sub-figures we have plotted, as the reference for comparison, linear functions of  $\alpha$. Thus, comparing slopes to the reference, we see that numerically we get order $1$ convergence for $t=0.3$, $t=0.4$ and $t=0.5$. However, for $t=0.6$, the rate of convergence is no more than $1/2$.
 }
\end{figure}


% show figures of errors in spectral space

==> numerics.tex <==
\section{Numerical implementation}\label{sec: numerics}
% \ADD{todo: add references}
{For numerical implementation, we choose to work in weaker spaces than what the wellposedness theorem dictates. Additionally we allow for boundary conditions in the numerical setup. We recognise these choices create gaps between the theory and the implementation.}

\subsection{Discretisation methods for $\alpha$--TQG and TQG   }\label{sec: numerics methods}

In this subsection, we describe the finite element (FEM) spatial discretisation, and finite difference Runge-Kutta time stepping discretisation methods that are utilised for the $\alpha$-TQG system. 
By setting $\alpha$ to zero we obtain our numerical setup for the TQG system. 

Consider a bounded domain $\domain$. Let $\p \domain$ denote the boundary. We impose Dirichlet boundary conditions
\begin{equation}\label{eq: tqg boundary conditions numerical}
    \psi^\alpha = 0, \    
    \Delta \psi^\alpha = 0, \qquad \text{on } \p \domain.
\end{equation}
For $\domain = \mathbb T^2$, our numerical setup does not change, in which case the boundary flux terms in the discretised equations are set to zero.

\subsubsection{The stream function equation}\label{sec: stream function discretisation}

Let $H^{1}\left(\domain\right)$ denote the Sobolev $W^{1,2}\left(\domain\right)$
space and let $\left\Vert .\right\Vert _{\partial\domain}$ denote
the $L^{2}\left(\partial\domain\right)$ norm. 
Define the space 
\begin{equation}\label{eq: w1 space}
    W^{1}\left(\domain\right):=\left\{ \nu\in H^{1}\left(\domain\right)\left|\left\Vert \nu\right\Vert _{\partial\domain}=0\right.\right\}.
\end{equation}
We express \eqref{constrtAlpha} as two inhomogeneous Helmholtz equations
\begin{align}
    \omega^\alpha - f &= (\Delta -1 ) \tilde\psi \label{eq:inhomogeneousHelmholtz}\\
    -\tilde\psi &= (\alpha \Delta - 1)\psi^\alpha\label{eq:inhomogeneousHelmholtzAlpha}. 
\end{align}
We take $\tilde\psi,\psi^\alpha \in W^1 (\domain)$.
Since the two equations are of the same form, let us first consider \eqref{eq:inhomogeneousHelmholtz}.
Using an arbitrary test function $\phi \in W^1(\domain)$, we obtain the following weak form of \eqref{eq:inhomogeneousHelmholtz},
\begin{align}
\langle\nabla \tilde\psi,\nabla\phi\rangle_\domain +\langle\tilde\psi,\phi\rangle_\domain  &=  -\langle \omega^\alpha - f, \phi \rangle_\domain.
\label{eq: inhomogeneousHelmholtz weak}
\end{align}
Define the functionals
\begin{align}
    L_\alpha(v, \phi) &:= \alpha\langle \nabla v, \nabla \phi \rangle_\domain +\langle v, \phi  \rangle_\domain \label{eq: psi bilinear form}\\
    F_{\cdot}(\phi) &:=  -\langle  \cdot, \phi \rangle_\domain
    \label{eq: psi linear form}
\end{align}
for $v, \phi \in W^1(\domain)$, then \eqref{eq: inhomogeneousHelmholtz weak} can be written as
\begin{equation}\label{eq: TQG weak elliptic}
    L_1(\tilde\psi, \phi) = F_{\omega^\alpha -  f^\alpha}(\phi).
\end{equation}
And similarly for \eqref{eq:inhomogeneousHelmholtzAlpha}, we have
\begin{equation}\label{eq: TQG weak elliptic alpha} 
    L_\alpha(\psi^\alpha, \phi) = F_{-\tilde\psi}(\phi).
\end{equation}
We discretise equations \eqref{eq: TQG weak elliptic} and \eqref{eq: TQG weak elliptic alpha} using a continuous
Galerkin (CG) discretisation scheme. 

Let $\delta$ be the discretisation parameter, and let $\domain_\delta$ denote a space filling triangulation of the domain, that consists of geometry-conforming nonoverlapping elements.
%Let $X_\delta^k$ denote the finite element space that consists of continuous functions, and including at least all polynomials of degree $k$ on each cell of $\domain_\delta$. 
Define the approximation space
% \begin{equation}
%     W^k_\delta = W^1(\domain) \cap X_\delta^k
% \end{equation}
% where $X_\delta^k$ is a finite element space consisting of continuous functions and including at least all polynomials of degree $k$ on each element of a triangulation $\domain_\delta$. More specifically, we have 
\begin{equation} \label{eq: cg space}
    W_\delta^{k}(\domain):=\left\{ \phi_\delta\in W^{1}\left(\domain\right)\ : \ \phi_\delta\in C\left(\domain\right),\left.\phi_\delta\right|_{K}\in\Pi^{k}\left(K\right)\text{ each } K \in \domain_\delta\right\}.
\end{equation}
in which $C(\domain)$ is the space of continuous functions on $\domain$, and  $\Pi^{k}\left(K\right)$ denotes the space of polynomials of degree at most $k$ on element $K\in \domain_\delta$. 

For \eqref{eq: TQG weak elliptic}, given $f_\delta \in W_\delta^k(\domain)$ and $\omega_\delta \in V_\delta^k(\domain)$ (see \eqref{DG space} for the definition of $V_\delta^k(\domain)$), 
our numerical approximation is the solution $\tilde\psi_\delta \in W_\delta^k(\domain)$ that satisfies 
\begin{equation}
L_1(\tilde\psi_\delta, \phi_\delta) = F_{\omega_\delta - f_\delta}(\phi_\delta)
\label{eq: TQG psi eqn weak discretised}
\end{equation}
for all test functions $\phi_\delta \in W_\delta^k(\domain)$. Then, using $\tilde\psi_\delta$, our numerical approximation of $\psi^\alpha$ is the solution $\psi_\delta^\alpha\in W_\delta^k(\domain)$ that satisfies
\begin{equation}\label{eq: TQG psi alpha eqn weak discretised}
L_\alpha(\psi_\delta^\alpha, \phi_\delta) = F_{-\tilde\psi_\delta} (\phi_\delta)
\end{equation}
for all test functions $\phi_\delta \in W_\delta^k(\domain)$.

 For a detailed exposition of the numerical algorithms that solves the discretised problems \eqref{eq: TQG psi eqn weak discretised} and \eqref{eq: TQG psi alpha eqn weak discretised} we point the reader to \cite{Gibson2019, Brenner2008}.

\subsubsection{Hyperbolic equations}\label{sec: buoyancy equation discretisation}
We choose to discretise the hyperbolic buoyancy \eqref{ceAlpha} and potential vorticity \eqref{meAlpha} equations using a discontinuous Galerkin (DG) scheme. For a detailed exposition of DG methods, we refer the interested reader to \cite{Hesthaven2008}.

Define the DG approximation space, denoted by $V_\delta^k(\domain)$, to be the element-wise polynomial space,
\begin{equation}\label{DG space}
    V_\delta^k(\domain) = \left\{ \left. v_\delta \in L^2(\domain) \right|\forall K \in \domain_\delta,\ \exists\phi_\delta\in \Pi^k (K):\ \left.v_\delta\right|_{K}=\left.\phi_\delta\right|_K\right\}.
\end{equation}
We look to approximate $b^\alpha$ and $\omega^\alpha$ in the space $V_\delta^k(\domain)$. Essentially, this means our approximations of $b^\alpha$ and $\omega^\alpha$ are each an direct sum over the elements in $\domain_\delta$. Additional constraints on the numerical fluxes across shared element boundaries are needed to ensure conservation properties and stability. 
Further, note that $W^k_\delta(\domain) \subset V^k_\delta(\domain)$. This inclusion is also needed for ensuring numerical conservation laws, see Section \ref{sec: numerics numerical conservation}.

For the buoyancy equation \eqref{ceAlpha}, we obtain the following variational formulation
\begin{align}
\langle \p_t b^\alpha, \nu_\delta \rangle _{K} & = \langle b^\alpha {\bf u}^\alpha,\nabla\nu_\delta\rangle _K - \langle b^\alpha {\bf u}^\alpha\cdot\normal,\nu_\delta\rangle _{\partial K},\quad K\in \domain_\delta
\label{eq: TQG b alpha equation weak}
\end{align}
where $\nu_\delta\in V^k_\delta(\domain)$ is any test function, $\p K$ denotes the boundary of $K$, and $\normal$ denotes the unit normal vector to $\p K$. Let $b^\alpha_\delta$ be the approximation of $b^\alpha$ in $V_\delta^k$, and let $\bu^\alpha_\delta = \nabla^\perp \psi^\alpha_\delta$ for $\psi^\alpha_\delta \in W^k_\delta$. Our discretised buoyancy equation over each element is given by
\begin{equation}
    \langle \p_t b^\alpha_\delta, \nu_\delta \rangle _{K} = \langle b^\alpha_\delta{\bf u}^\alpha_\delta,\nabla\nu_\delta\rangle _K - \langle b^\alpha_\delta{\bf u}^\alpha_\delta \cdot \normal,\nu_\delta\rangle _{\partial K}, \quad K \in \domain_\delta.
    \label{eq: TQG b alpha eqn weak discretised}
\end{equation}

Similarly, let $\omega^\alpha_\delta \in V_\delta^k(\domain)$ be the approximation of $\omega^\alpha$, and let $h_\delta \in W_\delta^k$. We obtain the following discretised variational formulation that corresponds to \eqref{meAlpha}, 
\begin{align}
\langle \p_t \omega^\alpha_\delta, \nu_\delta \rangle _{K} 
&= \langle (\omega^\alpha_\delta - b^\alpha_\delta){\bf u}^\alpha_\delta,\nabla\nu_\delta\rangle _{K}
-\langle (\omega^\alpha_\delta - b^\alpha_\delta) {\bf u}^\alpha_\delta \cdot\normal,\nu_\delta\rangle _{\partial K} \nonumber \\
& \qquad - \frac12\langle \nabla \cdot (b^\alpha_\delta \nabla^\perp h_\delta), \nu_\delta \rangle _K,
\qquad K\in \domain_\delta,
\label{eq: TQG omega alpha eqn weak discretised}
\end{align}
for test function $\nu_\delta \in V_\delta^k(\domain)$. 
% \begin{align}
% \langle\p_{t}\omega_\delta^\alpha,\nu_\delta
% \rangle_{K} 
% & =
% \langle(\omega^\alpha_\delta - b^\alpha_\delta) \nabla^{\perp} \psi_\delta,\nabla\nu_\delta\rangle_{K}-\langle\hat{f}_{\omega}(\omega_\delta^{+},\omega_\delta^{-},\nabla^{\perp}\psi_\delta\cdot\hat{n}),\nu_\delta^{-}\rangle_{\partial K}\nonumber \\
%  & \qquad-\frac{1}{2}\langle\nabla\cdot(b_\delta\nabla^{\perp}\rmh_\delta),\nu_\delta\rangle_{K}
% \label{eq: TQG omega eqn weak discretised}
% \end{align}

At this point, we only have the discretised problem on single elements. To obtain the global approximation, we sum over all the elements in $\domain_\delta$. In doing so, the $\p K$ terms in \eqref{eq: TQG b alpha eqn weak discretised} and \eqref{eq: TQG omega alpha eqn weak discretised} must be treated carefully.
Let $\p K_\text{ext}$ denote the part of cell boundary that is contained in $\p \domain$. Let $\p K_\text{int}$ denote the part of the cell boundary that is contained in the interior of the domain $\domain\backslash \p \domain$.
On $\p K_\text{ext}$ we simply impose the PDE boundary conditions. However, on $\p K_\text{int}$ we need to consider the contribution from each of the neighbouring elements.
By choice, the approximant $\psi^\alpha_\delta \in W_\delta^k$ is continuous on $\p K$. And since
\begin{equation}
    \bu^\alpha_\delta \cdot \normal = \nabla^\perp \psi^\alpha_\delta \cdot \normal = -\nabla \psi^\alpha_\delta \cdot \hat \tau = -\frac{\dd\psi^\alpha_\delta}{\dd\hat\tau},
\end{equation}
where $\hat\tau$ denotes the unit tangential vector to $\p K$, $\bu^\alpha_\delta \cdot \normal$ is also continuous. This means  $\bu^\alpha_\delta \cdot \normal$ in \eqref{eq: TQG b alpha eqn weak discretised} (also in \eqref{eq: TQG omega alpha eqn weak discretised}) is single valued. However, due to the lack of global continuity constraint in the definition of $V_k^\alpha(\domain)$, $b^\alpha_\delta$ and $\omega^\alpha_\delta$ are multi-valued on $\p K_\text{int}$. Thus, as our approximation of $\omega^\alpha$ and $b^\alpha$ over the whole domain is the sum over $K \in \domain_\delta$,  we have to constrain the flux on the set $\left(\bigcup_{K\in\domain_\delta} \p K \right)\setminus \p \domain$. This is done using appropriately chosen numerical flux fields in the boundary terms of \eqref{eq: TQG b alpha eqn weak discretised} and \eqref{eq: TQG omega alpha eqn weak discretised}.

Let 
{$\nu^{-}:=\lim_{\epsilon\uparrow0} \nu ({\bf x}+\epsilon\normal)$} 
and 
{ $\nu^{+}:=\lim_{\epsilon\downarrow0}\nu ({\bf x}+\epsilon\normal)$}, 
for ${\bf x}\in\partial K$, be the inside and outside (with respect to a fixed element $K$) values respectively, of a function $\nu$ on the boundary.
Let $\hat{f}$ be a \emph{numerical flux} function 
that satisfies the following properties:
\begin{enumerate}[(i)]
    \item consistency 
    \begin{equation}
     \hat f (\nu, \nu, \bu_\delta \cdot \normal) = \nu \bu_\delta\cdot\normal
     \label{eq: nflux consistency}
     \end{equation}
    
    \item conservative
    \begin{equation}
        \hat f (\nu^+, \nu^-, \bu_\delta\cdot \normal) = - \hat f (\nu^-, \nu^+, -\bu_\delta\cdot \normal)
        \label{eq: nflux conservative}
    \end{equation}
    
    \item $L^2$ stable in the enstrophy norm with respect to the buoyancy equation, see \cite[Section 6]{Bernsen2006}.
\end{enumerate}
% \CHANGE{Upwind scheme
% \[
% \hat{f} (b_\delta^{+},b_\delta^{-},{\bf u}\cdot\hat{n} )={\bf u}\cdot\hat{n}\begin{cases}
% b_\delta^{+} & \text{if }{\bf u}\cdot\hat{n}<0\\
% b_\delta^{-} & \text{if }{\bf u}\cdot\hat{n}\geq0.
% \end{cases}
% \]}
With such an $\hat f$, we replace 
$b^\alpha_\delta \bu^\alpha_\delta \cdot \normal$ by the numerical flux $\hat{f}(b_\delta^{\alpha, +},b_\delta^{\alpha, -},{\bf u}^\alpha_\delta \cdot\normal)$  in \eqref{eq: TQG b alpha eqn weak discretised}.
Similarly, in \eqref{eq: TQG omega alpha eqn weak discretised}, we replace $(\omega^\alpha_\delta - b^\alpha_\delta)\bu_\delta^\alpha \cdot \normal$ by $\hat{f}((\omega^\alpha_\delta - b^\alpha_\delta)^{+}, (\omega^\alpha_\delta - b^\alpha_\delta)^{-}, \bu_\delta^\alpha \cdot \normal)$.

\begin{remark}
For a general nonlinear conservation law, one has to solve what is called the \emph{Riemann problem} for the numerical flux, see \cite{Hesthaven2008} for details.
In our setup, we use the following local Lax-Friedrichs flux, which is an approximate Riemann solver,
\begin{equation}
\hat{f}(\nu^+, \nu^-, \bu_\delta\cdot\normal) = \bu_\delta\cdot\normal
\{\{ \nu  \}\} - \frac{|\bu_\delta\cdot\normal|}{2}\llbracket\nu\rrbracket
\end{equation}
where
\begin{equation}
\{\{\nu\}\}:=\frac{1}{2}(\nu^{-}+\nu^{+}),\qquad
\llbracket\nu\rrbracket:=\normal^{-}\nu^{-}+\normal^{+}\nu^{+}.
\end{equation}
\end{remark}

Finally, our goal is to find $b^\alpha_\delta, \omega^\alpha_\delta \in V_\delta^k(\domain)$ such that for all {$\nu_\delta\in V_\delta^k(\domain)$} we have
\begin{align}
\sum_{K\in \domain_\delta} \langle \p_t b^\alpha_\delta, \nu_\delta\rangle _{K} 
&=
\sum_{K\in \domain_\delta}
\big\{
\langle b^\alpha_\delta\nabla^{\perp} \psi^\alpha_\delta, \nabla \nu_\delta\rangle _{K}  -
\langle \hat{f}_{b^\alpha}(b_\delta^{\alpha, +},b_\delta^{\alpha, -},\nabla^{\perp}\psi^\alpha_\delta \cdot \normal), \nu_\delta^{-}\rangle _{\partial K}
\big\}, 
\label{eq: TQG b eqn weak discretised numerical flux}
\\
\sum_{K\in \domain_\delta} \langle \p_t \omega^\alpha_\delta, \nu_\delta \rangle _{K} 
&= 
\sum_{K\in \domain_\delta} 
\big\{
\langle (\omega^\alpha_\delta - b^\alpha_\delta)\nabla^{\perp}\psi^\alpha_\delta,\nabla\nu_\delta\rangle _{K} - \frac12\langle \nabla \cdot (b^\alpha_\delta \nabla^\perp h_\delta), \nu_\delta \rangle _K
\label{eq: TQG omega eqn weak discretised numerical flux}
% \\
% &\qquad\quad
% -\langle \omega^\alpha_\delta \nabla^\perp \psi^\alpha_\delta \cdot\normal,
% \nu_\delta^-
% \rangle _{\partial K_\text{ext}}
% \nonumber
\\
&\qquad -
\langle \hat{f}_{\omega^\alpha}((\omega^\alpha_\delta - b^\alpha_\delta)^{+}, (\omega^\alpha_\delta - b^\alpha_\delta)^{-}, \nabla^\perp \psi_\delta^\alpha \cdot \normal),
\nu_\delta^ -
\rangle _{\partial K}
\big\}
\nonumber
\end{align}
with $\psi_\delta^\alpha \in W_\delta^k(\domain)$ being the numerical approximation to the stream function. 

\begin{remark}
In \eqref{eq: TQG b eqn weak discretised numerical flux} and \eqref{eq: TQG omega eqn weak discretised numerical flux} we do not explicitly distinguish $\p K_\text{ext}$ and $\p K_\text{int}$ because for the boundary conditions \eqref{eq: tqg boundary conditions numerical}, the $\p K_\text{ext}$ terms vanish. 
\end{remark}


\subsubsection{Numerical conservation}
\label{sec: numerics numerical conservation}
Conservation properties of the TQG system was first shown in \cite{Holm2021}. More specifically, the TQG system conserves energy, and an infinite family of quantities called casimirs. Proposition \ref{prop: TQG alpha conservation} below describes the conservation properties of the $\alpha$--TQG system. We note that the form of the conserved energy and casimirs are the same as that of the TQG system.
Although the result is stated for the system with boundary conditions, it is easy to show that the same result holds for $\mathbb T^2$ .

\begin{proposition}[$\alpha$--TQG conserved quantities]\label{prop: TQG alpha conservation}
On a bounded domain $\domain$ with boundary $\p \domain$, consider the $\alpha$-TQG system \eqref{ceAlpha} -- \eqref{constrtAlpha} 
with boundary conditions
\begin{equation}\label{eq: tqg boundary conditions}
    \normal\cdot \bu^\alpha = 0, \  \normal\times \nabla b^\alpha = 0,\   
    \frac \dd {\dd t}
    \int_{\p \domain} \nabla \psi^\alpha \cdot \normal = 0, \ 
    \frac \dd {\dd t}
    \int_{\p \domain}  \nabla \Delta \psi^\alpha \cdot \normal = 0, \ 
    \normal \times \nabla \Delta \psi^\alpha = 0
\end{equation}
We have
\begin{equation}\label{eq: tqg energy}
     E^\alpha(t) := - \frac12  \int_\domain \{(\omega^\alpha - f)\psi^\alpha + \rmh b^\alpha \} \dd \bx,
\end{equation}
and
\begin{equation}\label{eq: tqg casimirs}
     C^\alpha_{\Psi, \Phi}(t) :=   \int_\domain \{ \Psi(b^\alpha) + \omega^\alpha \Phi(b^\alpha) \} \dd \bx ,\qquad \forall \Psi, \Phi \in C^\infty
\end{equation}
are conserved, i.e. $\dd_t E^\alpha(t) = 0$ and $\dd_t C^\alpha_{\Psi, \Phi}(t) = 0$.
\end{proposition}

\begin{proof}
For the energy $E^\alpha(t)$, we obtain
\begin{align*}
    \frac \dd {\dd t} E^\alpha(t) &= -\frac12 \frac \dd {\dd t} \int_\domain \{\psi^\alpha (\Delta - 1)(1-\alpha \Delta)\psi^\alpha + \rmh b^\alpha \} \dd \bx \\
    % &= -\frac12 \int_\domain \{\p_t \psi (\Delta -1)(1-\alpha\Delta)\psi + \psi (\Delta-1)(1-\alpha\Delta)\p_t \psi + h \p_t b \} \dd \bx \\
    &=\int_\domain \{-\psi^\alpha \ \p_t \omega^\alpha - \frac12 h \p_t b^\alpha \} \dd\bx.
\end{align*}
Substitute $\p_t \omega^\alpha$ and $\p_t b^\alpha$ using \eqref{ceAlpha} and \eqref{meAlpha},
the result then follows from direct calculations.

Similarly for the casimirs, we obtain the result by directly evaluating $\dd_t C^\alpha_{\Psi, \Phi}(t)$.
\end{proof}

\begin{remark}
In \eqref{eq: tqg boundary conditions}, except for the integral Neumann boundary conditions, we effectively have Dirichlet boundary conditions for $\psi^\alpha$, $b^\alpha$ and $\Delta \psi^\alpha$. The integral Neumann boundary conditions can be viewed as imposing the Kelvin theorem on the boundary -- consider
\begin{equation}
    \frac \dd {\dd t}
    \int_{\p \domain}  \nabla (\psi^\alpha - \alpha \Delta \psi^\alpha) \cdot \normal = 0,
\end{equation}
and apply the divergence theorem.

In our FEM discretisation, we impose only Dirichlet boundary conditions.
% as can be seen from the definition of the approximation space $W^k_\delta(\domain)$. 
If the integral Neumann boundary conditions are not imposed, then for Proposition \ref{prop: TQG alpha conservation} to hold, we necessarily require $\psi^\alpha$ and $\Delta \psi^\alpha$ on $\p \domain$ to be \emph{zero}.
\end{remark}

We now analyse the conservation properties of our spatially discretised $\alpha$-TQG system. 
Let $\langle \cdot, \cdot \rangle_{H^1(\domain)}$ be the $H^1(\domain)$ inner product.
Define the numerical total energy
\begin{equation}\label{eq: numerical energy}
    E^\alpha_\delta(t) = 
    \frac12
    \langle \psi^\alpha_\delta
    , \tilde \psi_\delta
    \rangle_{H^1(\domain)}
    % L_1(\psi^\alpha_\delta, \tilde\psi_\delta)
    - 
    \frac12 
    \langle \rmh_\delta, b^\alpha_\delta \rangle_\domain,
\end{equation}
% \CHANGE{CHECK: If $\rmh_h \in W_h^k$ and $b_h \in V_h^k$, how is $\langle \rmh_h, b_h \rangle_\Omega$ defined? If $W_h^k \subset V_h^k$ then it's ok.}
in which $\psi_\delta^\alpha, \tilde{\psi}_\delta \in W_\delta^\alpha(\domain)$ and $b_\delta^\alpha\in V_\delta^k(\domain)$ are the numerical approximations of $\psi^\alpha$, $\tilde{\psi}$ and $b^\alpha$ respectively.
Define the numerical casimir functional
\begin{equation}\label{eq: TQG numerical casimirs}
C_{\delta}^\alpha(t; \Psi, \Phi ):= \langle\Psi(b_\delta^\alpha),1 \rangle_\domain
+ \langle \omega_\delta^\alpha \Phi(b_\delta^\alpha) \rangle_\domain, 
\quad \Psi, \Phi \in C^\infty.
\end{equation}

\begin{lemma} 
With boundary conditions \eqref{eq: tqg boundary conditions numerical}
\begin{equation}
    \frac \dd {\dd t} E^\alpha_\delta(t) = 0
\end{equation}
for $\alpha = 0$.
\end{lemma}
In other words, the semi-discrete discretisation conserves energy in the TQG case.
\begin{proof}
We consider $\dd/\dd_t$ evaluated at an arbitrary fixed value $t_0$.
First note that when $\alpha=0$, we have $\psi^\alpha_\delta = \tilde \psi_\delta$. Then, from \eqref{eq: psi bilinear form} we have
\begin{align}
    2E_\delta^\alpha(t) 
    % &=  L_1(\psi_\delta^\alpha, \tilde{\psi}_\delta) - \langle \rmh_\delta, b_\delta^\alpha \rangle_\Omega \nonumber \\
    &= L_1 (\psi_\delta^\alpha, {\psi}^\alpha_\delta) - \langle \rmh_\delta, b_\delta^\alpha \rangle_\Omega
    \label{eq: TQG total energy numerical}
\end{align}
% Differentiating the first term with respect to time, we get 
% \begin{equation}
% \frac \dd {\dd t}\Big|_{t=t_0} L_1(\psi^\alpha_\delta, \tilde{\psi}_\delta) = L_1(\p_t \psi^\alpha_\delta, \tilde{\psi}_\delta)\big|_{t=t_0}
% + L_1(\psi^\alpha_\delta, \p_t \tilde{\psi}_\delta)\big|_{t=t_0}.
% \end{equation}
For the first term in \eqref{eq: TQG total energy numerical}, following \eqref{eq: TQG psi eqn weak discretised} we have
\begin{align}
    % \left.\frac \dd {\dd t}\right|_{t=t_0} L_1(\tilde\psi_\delta, \phi_\delta) = 
    % \left.L_1(\p_t \tilde\psi_\delta, \phi_\delta)\right|_{t=t_0} 
    % &= \left.\frac \dd {\dd t}\right|_{t=t_0} F_{\omega^\alpha_\delta - f^\alpha_\delta}(\phi_\delta) = - \left.\langle\p_t \omega^\alpha_\delta, \phi_\delta \rangle_\domain \right|_{t=t_0} 
    % \nonumber \\
    \left.L_1(\p_t \psi_\delta, \phi_\delta)\right|_{t=t_0} = - \sum_{K\in \mathcal \domain_\delta} \left.\langle\p_t \omega^\alpha_\delta, \phi_\delta \rangle_K \right|_{t=t_0},
    \quad 
    \forall \phi_\delta \in W_\delta^k(\domain).
    % \nonumber
\end{align}
% in which the test function $\phi_\delta \in W_\delta^k(\domain)$ is arbitrary. 
 Thus, substituting in the discretised equation \eqref{eq: TQG omega eqn weak discretised numerical flux} for $\omega^\alpha$, we obtain
\begin{align}
    % - L_1(\left.\p_t \tilde\psi_\delta, \phi_\delta)\right|_{t=t_0}
    - L_1(\left.\p_t \psi_\delta, \phi_\delta)\right|_{t=t_0}
    % &= 
    % \sum_{K\in \mathcal T_\delta} 
    % \big[\langle \omega_\delta \nabla^\perp \psi_\delta, \nabla\phi_\delta\rangle _{K}
    % - \langle \hat f_1(\omega^+_\delta,\omega^-_\delta, \nabla^\perp \psi_\delta\cdot\hat{n}),\phi_\delta^-\rangle _{\partial K} \nonumber \\
    % & \qquad 
    % + \langle b_\delta \nabla^\perp(\frac12 \rmh_\delta-\psi_\delta),\nabla\phi_\delta\rangle _K 
    % \nonumber \\
    % &\qquad
    % -\langle \hat f_2(b^+, b^-, \nabla^\perp (\frac12 \rmh_\delta - \psi_\delta)\cdot \normal ), \phi_\delta^-\rangle_{\p K} \big]_{t=t_0}.
    % \\
    % \sum_{K\in \domain_\delta} \langle \p_t \omega^\alpha_\delta, \nu_\delta \rangle _{K} 
&= 
\sum_{K\in \domain_\delta} 
\left[
\big\{
\langle (\omega^\alpha_\delta - b^\alpha_\delta)\nabla^{\perp}\psi^\alpha_\delta,\nabla\phi_\delta\rangle _{K} - \frac12\langle \nabla \cdot (b^\alpha_\delta \nabla^\perp h_\delta), \phi_\delta \rangle _K
\right.
% \\
% &\qquad\quad
% -\langle \omega^\alpha_\delta \nabla^\perp \psi^\alpha_\delta \cdot\normal,
% \phi_\delta^-
% \rangle _{\partial K_\text{ext}}
\nonumber
\\
&\qquad -
\left.
\langle \hat{f}_{\omega^\alpha}((\omega^\alpha_\delta - b^\alpha_\delta)^{+}, (\omega^\alpha_\delta - b^\alpha_\delta)^{-}, \nabla^\perp \psi_\delta^\alpha \cdot \normal),
\phi_\delta^ -
\rangle _{\partial K}
\big\}
\right]_{t=t_0},
\label{eq: TQG kinetic energy time differential}
\end{align}
in which 
% \eqref{eq: TQG kinetic energy time differential}, 
we can choose $\phi_\delta=[\psi^\alpha_\delta]_{t=t_0}$. This choice is consistent with the discretisation space $V_\delta^k(\domain)$ for $\omega^\alpha$, since $W_\delta^k(\domain) \subset V_\delta^k(\domain)$.
% {\color{red} (Not true, need more regularity) We also have $L_1(\phi, \tilde\psi_\delta) = L_1((1-\alpha\Delta)\phi, \psi_\delta),$ $\phi,\psi_\delta, \tilde \psi_\delta \in W_\delta^k(\domain)$}. 
% Further, assuming $\p_t \psi_\delta \in W_\delta^k(\domain)$, we get ${\color{red} \left.L_1(\p_t \psi_\delta^\alpha, \tilde\psi_\delta)\right|_{t=t_0} = \left.L_1(\p_t \tilde \psi_\delta, \psi_\delta)\right|_{t=t_0}}$.

Similarly, for the second term in \eqref{eq: TQG total energy numerical}, using \eqref{eq: TQG b eqn weak discretised numerical flux} we obtain
\begin{equation}
    \left.\frac \dd {\dd t}\right\vert_{t=t_0} \langle b^\alpha_\delta, \nu_\delta \rangle_\domain
    % &= \sum_{K\in  \domain_\delta} \langle \p_t b^\alpha_\delta, \nu_\delta \rangle_K \big\vert_{t=t_0}
    % \nonumber \\
    = \sum_{K\in \domain_\delta} \left[ 
    \big\{
        \langle b^\alpha_\delta\nabla^{\perp} \psi^\alpha_\delta, \nabla \nu_\delta\rangle _{K}  -
        \langle \hat{f}_{b^\alpha}(b_\delta^{\alpha, +},b_\delta^{\alpha, -},\nabla^{\perp}\psi^\alpha_\delta \cdot \normal), \nu_\delta^{-}\rangle _{\partial K}
    \big\}
    \right]_{t=t_0},
    \label{eq: TQG potential energy time differential}
\end{equation}
where we can choose $\nu_\delta = \rmh_\delta$.

Putting together \eqref{eq: TQG total energy numerical}, \eqref{eq: TQG kinetic energy time differential} and \eqref{eq: TQG potential energy time differential}, and substituting in $\rmh_\delta$ and $[\psi^\alpha_\delta]_{t=t_0}$ for the arbitrary choices, we obtain
\begin{align}
    2 \frac \dd {\dd t}\Big|_{t=t_0} E^\alpha_\delta(t)
    &= 
    - \sum_{K\in \domain_\delta} 
    \left[
    2 \Big\{
    \langle (\omega^\alpha_\delta - b^\alpha_\delta)
    \underbrace{
    \nabla^{\perp}
    \psi^\alpha_\delta,\nabla
    \psi^\alpha_\delta
    }_{=0}
    \rangle _{K} - \frac12\langle \nabla \cdot (b^\alpha_\delta \nabla^\perp h_\delta), \psi^\alpha_\delta
    \rangle _K
    \right.
    % \right.
    \nonumber
    \\
    &\qquad 
    -
    % \left.
    \left.
    \langle \hat{f}_{\omega^\alpha}((\omega^\alpha_\delta - b^\alpha_\delta)^{+}, (\omega^\alpha_\delta - b^\alpha_\delta)^{-}, \nabla^\perp \psi_\delta^\alpha \cdot \normal),
    {\psi^\alpha_\delta}^-
    \rangle _{\partial K}
    \Big\}
    \right.
    % \right]_{t=t_0}
    \nonumber
    % \\
    % & \qquad {\color{red} + L_1(\p_t \psi_\delta^\alpha, \tilde\psi_\delta)}
    % \nonumber
    \\
    & 
    % -\sum_{K\in \domain_\delta} 
    +
    \left. 
    %\left[
    \Big\{
        \underbrace{
        \langle
        b^\alpha_\delta\nabla^{\perp} \psi^\alpha_\delta, \nabla \rmh_\delta\rangle _{K}  
        }_{=- \langle
        b^\alpha_\delta\nabla^{\perp}
        \rmh_\delta, \nabla \psi^\alpha_\delta\rangle _{K}  }
        -
        \langle \hat{f}_{b^\alpha}(b_\delta^{\alpha, +},b_\delta^{\alpha, -},\nabla^{\perp}\psi^\alpha_\delta \cdot \normal), \rmh_\delta^{-}\rangle _{\partial K}
    \Big\}
    \right]_{t=t_0}
\end{align}
% \begin{align}
%     2 \frac d {dt}\Big|_{t=t_0} E_\delta(t) &= \sum_{K\in \mathcal T_\delta} 
%     \Big[
%     2 \underbrace{\langle \omega_\delta \nabla^\perp \psi_\delta, \nabla\psi_\delta\rangle _{K}}_{=0}
%     -2  \langle \hat f_1(\omega^+_\delta,\omega^-_\delta, \nabla^\perp \psi_\delta\cdot\hat{n}),\psi_\delta^-\rangle _{\partial K}
%     \nonumber \\
%     & \qquad 
%     + 2 \langle b_\delta \nabla^\perp(\frac12 \rmh_\delta\underbrace{-\psi_\delta),\nabla\psi_\delta}_{\text{gives $0$}}\rangle _K 
%     \nonumber \\
%     &\qquad
%     -2 \langle \hat f_2(b^+, b^-, \nabla^\perp (\frac12 \rmh_\delta - \psi_\delta)\cdot \normal ), \psi_\delta^-\rangle_{\p K} \nonumber \\
%     & \qquad 
%     + \langle b_\delta\nabla^{\perp}\psi_\delta, \nabla \rmh_\delta\rangle _{K}  -
%     \langle \hat{f}(b_\delta^{+},b_\delta^{-},\nabla^{\perp}\psi_\delta \cdot \hat{n}), \rmh_\delta^{-}\rangle _{\partial K} \Big]_{t=t_0}
%     \\
%     &= \sum_{K\in \mathcal T_\delta} 
%     \Big[
%     \langle b_\delta \nabla^\perp\rmh_\delta,\nabla\psi_\delta\rangle _K 
%     + \underbrace{\langle b_\delta\nabla^{\perp}\psi_\delta, \nabla \rmh_\delta\rangle _{K}}
%     _{= - \langle b_\delta \nabla^\perp \rmh_\delta, \nabla \psi_\delta\rangle_K}
%     \nonumber \\
%     & \qquad 
%     - 2 \langle \hat f_1(\omega^+_\delta,\omega^-_\delta, \nabla^\perp \psi_\delta\cdot\hat{n}),\psi_\delta^-\rangle _{\partial K}
%     \nonumber \\
%     &\qquad
%     -2 \langle \hat f_2(b^+, b^-, \nabla^\perp (\frac12 \rmh_\delta - \psi_\delta)\cdot \normal ), \psi_\delta^-\rangle_{\p K} \nonumber \\
%     & \qquad 
%     - \langle \hat{f}(b_\delta^{+},b_\delta^{-},\nabla^{\perp}\psi_\delta \cdot \hat{n}), \rmh_\delta^{-}\rangle _{\partial K} \Big]_{t=t_0}
% \end{align}
% Hence
\begin{align}
    \frac \dd {\dd t} E^\alpha_\delta(t) &= \sum_{K\in \mathcal \domain_\delta} 
    \Big[
    - \langle \hat f_{\omega^\alpha}((\omega^\alpha_\delta-b^\alpha_\delta)^+,(\omega_\delta^\alpha - b^\alpha_\delta)^-, \nabla^\perp \psi^\alpha_\delta\cdot\normal),{\psi^\alpha_\delta}^-\rangle _{\partial K}
    \nonumber \\
    % &\qquad
    % -2 \langle \hat f_2(b^+_\delta, b^-_\delta, \nabla^\perp (\frac12 \rmh_\delta - \psi_\delta)\cdot \normal ), \psi_\delta^-\rangle_{\p K} \nonumber \\
    & \qquad 
    - \frac12
    \langle \hat{f}_{b^\alpha}({b^\alpha_\delta}^{+},{b^\alpha_\delta}^{-},\nabla^{\perp}\psi^\alpha_\delta \cdot \normal), \rmh_\delta^{-}\rangle _{\partial K} \Big]_{t=t_0}
    \label{eq: numerical energy temp}
\end{align}
Since $\psi_\delta$ and $\rmh_\delta$ are continuous across element boundaries, we have $\psi_\delta^+ = \psi_\delta^-$ and $\rmh_\delta^+ = \rmh_\delta^-$.
Thus, if the numerical fluxes $\hat f_{\omega^\alpha}$ and $\hat f_{b^\alpha}$ satisfy the conservative property \eqref{eq: nflux conservative}, the sum of flux terms is zero.
\end{proof}

\begin{remark}
In order for our semi-discrete discretisation to conserve numerical energy when $\alpha > 0$, more regularity is required for the approximation space for $\psi^\alpha_\delta$. Additionally, the current scheme coupled with the time stepping algorithm do not conserve  casimirs. For future work, we look to explore casimir conserving schemes for the model.
\end{remark}

% \begin{lemma}

% \end{lemma}


\subsubsection{Time stepping}
% For the time stepping scheme, we follow \cite{gottlieb2005high} and
% use a strong stability preserving Runge Kutta method of order 3 (SSPRK3)
% with the  Courant--Friedrich--Lewy (CFL) condition being $1/3.$
To discretise the time derivative, we use the strong stability preserving Runge-Kutta of order 3 (SSPRK3) scheme, see \cite{Hesthaven2008}.
Writing the finite element spatial discretisation formally as 
\begin{equation}
    \partial_{t}b^\alpha_\delta={\rm f}_\delta(b^\alpha_\delta)
\end{equation}
where ${\rm f}_\delta$ is the discretisation operator that follows from \eqref{eq: TQG b eqn weak discretised numerical flux}, and
\begin{equation}
     \partial_t \omega = {\rm g}_\delta (\omega, b)
\end{equation}
where ${\rm g}_\delta$ is the discretisation operator that follows from \eqref{eq: TQG omega eqn weak discretised numerical flux}.
Let $b^{\alpha, n}_\delta$ and $\omega^{\alpha,n}_\delta$ denote the approximation of $b^\alpha_\delta$ and $\omega^\alpha_\delta$ at time step $t_n$.
The SSPRK3
time discretisation is as follows 
\begin{subequations}
\begin{align}
    b^{(1)} & = b^{\alpha,n}_\delta + \Delta t \ {\rm f}_\delta (b^{\alpha,n}_\delta)\\
	\omega^{(1)} & =\omega^{\alpha,n}_\delta+\Delta t \  {\rm g}_\delta\left(\omega^{\alpha,n}_\delta, b^{\alpha,n}_\delta \right)\\
	b^{\left(2\right)} 
	&=\frac{3}{4}b^{\alpha,n}_\delta +\frac{1}{4}\left(b^{\left(1\right)}+\Delta t \ {\rm f}_\delta\left(b^{\left(1\right)}\right)\right)\\
	\omega^{\left(2\right)} 
	&= \frac{3}{4}\omega^{\alpha,n}_\delta
	+\frac{1}{4}\left(\omega^{\left(1\right)}+\Delta t \  {\rm g}_\delta\left(\omega^{\left(1\right)}, b^{(1)}\right)\right)\\
	b^{\alpha,n+1}_\delta & =\frac{1}{3}b^{\alpha,n}_\delta+\frac{2}{3}\left(b^{\left(2\right)}+\Delta t \  {\rm f}_\delta\left(b^{\left(2\right)}\right)\right)\\
	\omega^{\alpha,n+1}_\delta & =\frac{1}{3}\omega^{\alpha,n}_\delta
	+\frac{2}{3}\left(\omega^{\left(2\right)}+\Delta t \  {\rm g}_\delta\left(\omega^{\left(2\right)}, b^{(2)}\right)\right)
\end{align}
\end{subequations}
where $\Delta t = t_{n+1}-t_{n}$ each $n$. 

% \begin{align*}
%     b^{(1)} & = b^n + \Delta f_\delta (b^n)
%     \\
% 	\omega^{(1)} & =\omega^{n}+\Delta g_\delta\left(\omega^{n}, b^n\right)
% 	\\
% 	b^{\left(2\right)} 
% 	&=\frac{3}{4}b^{n}+\frac{1}{4}\left(b^{\left(1\right)}+\Delta f_\delta\left(b^{\left(1\right)}\right)\right)
% 	\\
% 	& = \frac{3}{4}b^{n}+
% 	\frac{1}{4}b^n + \frac{1}{4}\Delta f_h (b^n)+
% 	\frac{1}{4}\Delta 
% 	f_\delta\left(b^n + \Delta f_h (b^n)\right)
% 	\\
% 	&= b^{n}+
% 	\frac{1}{4}\Delta f_h (b^n)+
% 	\frac{1}{4}\Delta 
% 	f_\delta(b^{(1)})
% 	\\
% 	\omega^{\left(2\right)} & =\frac{3}{4}\omega^{n}+\frac{1}{4}\left(\omega^{\left(1\right)}+\Delta g_\delta\left(\omega^{\left(1\right)}, b^{(1)}\right)\right)
% 	\\
% 	& =
% 	\frac{3}{4}\omega^{n}+\frac{1}{4}\Big[\omega^{n}+\Delta g_\delta\left(\omega^{n}, b^n\right)+\Delta g_\delta\big(
% 	\omega^{(1)},
% 	b^{(1)}\big)\Big]
% 	\\
% 	& =
% 	\omega^{n} + \frac14\Big[\Delta g_\delta\left(\omega^{n}, b^n\right)+\Delta g_\delta\big(
% 	\omega^{(1)},
% 	b^{(1)}\big)\Big]
% % 	\\
% % 	& =
% % 	\omega^{n} + \frac14\Big[
% % 	2\Delta g_\delta\left(\omega^{n}, b^n\right)
% % 	+ \Delta^2 g(\omega^n, b^n) g_h_x(\omega^n , b^n)
% % 	+ \Delta^2 f_h(b^n) g_h_y(\omega^n, b^n) +O(\Delta^3)
% % 	]
% 	\\
% 	& = 
% 	\omega^{n} + \frac12
% 	\Delta g_\delta\left(\omega^{n}, b^n\right)
% 	+ O(\Delta^2)
% 	\\
% 	b^{n+1} & =\frac{1}{3}b^{n}+\frac{2}{3}
% 	\left(b^{\left(2\right)}
% 	+\Delta f_\delta\left(b^{\left(2\right)}\right)\right)
% 	\\
% 	&=b^{n}
% 	+ 
% 	\left(
% 	\frac16\Delta f_h (b^n)+
% 	\frac16\Delta 
% 	f_\delta(b^{(1)})
% 	+
% 	\frac23\Delta f_\delta
% 	\left(
% 	b^{\left(2\right)}
% 	\right)\right)
% 	\\
% 	&=
% 	b^{n}
% 	+ 
% 	\left(
% 	\frac13\Delta f_h (b^n)
% 	+ \frac16\Delta^2 f_h'(b^n) f_h(b^n) + O(\Delta^3)
% 	\right.\\
% 	&
% 	\left.
% 	+
% 	\frac23\Delta f_\delta
% 	(
% 	b^{n}+
% 	\frac{1}{4}\Delta f_h (b^n)+
% 	\frac{1}{4}\Delta 
% 	f_\delta(b^{(1)})
% 	)
% 	\right)
% 	\\
% 	&= b^n + \Delta f_h(b^n) + O(\Delta^2)
% 	\\
% 	\omega^{n+1} & =\frac{1}{3}\omega^{n}+\frac{2}{3}\left(\omega^{\left(2\right)}+\Delta g_\delta\left(\omega^{\left(2\right)}, b^{(2)}\right)\right)
% 	\\
% 	& =
% 	\frac{1}{3}\omega^{n}
% 	+
% 	\frac{2}{3}
% 	\left(
% 	\omega^{n} + \frac12
% 	\Delta g_\delta\left(\omega^{n}, b^n\right)
% 	+ O(\Delta^2)\right.
% 	\\
% 	& + \left. \Delta g_\delta
% 	\left(\omega^{n} + \frac12
% 	\Delta g_\delta\left(\omega^{n}, b^n\right)
% 	+ O(\Delta^2), b^{n}+
% 	\frac{1}{4}\Delta f_h (b^n)+
% 	\frac{1}{4}\Delta 
% 	f_\delta(b^{(1)})\right)\right)
% 	\\
% 	& =
% 	\omega^{n}
% 	+
% 	\frac{2}{3}
% 	\left(
% 	\frac12
% 	\Delta g_\delta\left(\omega^{n}, b^n\right)
% 	 + \Delta 
% 	g_\delta(\omega^n, b^n)+ O(\Delta^2)
% 	\right)
% 	\\
% 	& = \omega^n + \Delta g_h(\omega^n, b^n) + O(\Delta^2)
% \end{align*}

% In variational form, we have

% \begin{align}\left\langle v_\delta,\omega^{(1)}\right\rangle _{K} 
% & =\left\langle v_\delta,\omega^{n}\right\rangle _{K}
% -\Delta t
% \left(
% \left\langle \nabla v_\delta,-(\omega^{n}-b^n)\nabla^{\perp}\psi_\delta^{n}\right\rangle _{K}+\left\langle v_\delta,\omega^{n}\nabla^{\perp}\psi_\delta^{n}\cdot\hat{n}\right\rangle _{\partial K}
% \right)
% \nonumber
% \\
% & - \Delta t 
% \left(  
% \left\langle \nabla v_\delta,-b^{n}\nabla^{\perp}\rmh_\delta^{n}\right\rangle _{K}+\left\langle v_\delta,b^{n}\nabla^{\perp}\rmh_\delta^{n}\cdot\hat{n}\right\rangle _{\partial K}
% \right)
% \\
% \dots &
% % \left\langle v_\delta,\omega^{\left(2\right)}\right\rangle _{K} & =\frac{3}{4}\left\langle v_\delta,\omega^{n}\right\rangle _{K}+\frac{1}{4}\left\langle v_\delta,\omega^{\left(1\right)}\right\rangle _{K}\\
% % & \qquad-\frac{\Delta t}{4}\left(\left\langle \nabla v_\delta,-\omega^{\left(1\right)}\nabla^{\perp}\psi_\delta^{\left(1\right)}\right\rangle _{K}+\left\langle v_\delta,\omega^{\left(1\right)}\nabla^{\perp}\psi_\delta^{\left(1\right)}\cdot\hat{n}\right\rangle _{\partial K}\right)\\
% % \left\langle v_\delta,\omega^{n+1}\right\rangle _{K} & =\frac{1}{3}\left\langle v_\delta,\omega^{n}\right\rangle _{K}+\frac{2}{3}\left\langle v_\delta,\omega^{\left(2\right)}\right\rangle _{K}\\
% % & \qquad-\frac{2\Delta t}{3}\left(\left\langle -\omega^{\left(2\right)}\nabla^{\perp}\psi_\delta^{\left(2\right)},\nabla v_\delta\right\rangle _{K}+\left\langle v_\delta,\omega^{\left(2\right)}\nabla^{\perp}\psi_\delta^{\left(2\right)}\cdot\hat{n}\right\rangle _{\partial K}\right)
% \end{align}
% for each $K\in\mathcal{T}_\delta.$ 


\subsection{$\alpha$-TQG linear thermal Rossby wave stability analysis}\label{sec: numerics linear stability analysis}

% The regularised TQG model is
% \begin{align}
% \p_{t}b+\nabla\cdot(b\tilde{\bu}) & =0\\
% \p_{t}\omega+\nabla\cdot(\omega\tilde{\bu}) & =\nabla\cdot\left(b\tilde{\bu}-\frac{1}{2}b\nabla^{\perp}\rmh\right)\\
% \tilde{\bu} & =\nabla^{\perp}\tilde{\psi}\\
% \bu & =\nabla^{\perp}\psi\\
% \omega & =(\Delta-1)\psi+f.\\
% \psi & =(1-\alpha^{2}\Delta)\tilde{\psi}
% \end{align}

A dispersion relation for the TQG system was derived in \cite{Holm2021}. There, the authors showed that the linear thermal Rossby waves of the TQG system possess high wavenumber instabilities. More specifically, the Doppler-shifted phase speed of these waves becomes complex at sufficiently high wavenumbers. However, the growth rate of the instability decreases to zero as $|\bk|^{-1}$, in the limit that $|\bk|\to\infty$. Consequently, the TQG dynamics is linearly well-posed in the sense of Hadamard. That is, the TQG solution depends continuously on initial conditions. 
In this subsection, using the same equilibrium state as in \cite{Holm2021}, we derive a dispersion relation for the  thermal Rossby wave solutions of the linearised $\alpha$-TQG system. Again the Doppler-shifted phase speed of these waves becomes complex at sufficiently high wavenumbers. However, in this case, the growth rate of the instability decreases to zero as $|\bk|^{-2}$, in the limit that $|\bk|\to\infty$. In the limit that $\alpha$ tends to zero, one recovers the TQG dispersion relation derived in \cite{Holm2021}.

For the reader's convenience, we repeat the equations solved by the pair of variables $(b^\alpha,\omega^\alpha)$ in the $\alpha$-TQG system in \eqref{ceAlpha}--\eqref{meAlpha}, as formulated now in vorticity-streamfunction form with fluid velocity given by ${\bu}^\alpha =\nabla^\perp \psi^\alpha$. This formulation is given by
\begin{align}
\frac{\partial}{\partial t} b^\alpha + J(\psi^\alpha,b^\alpha) &= 0,
\label{ceZero-redux}\\
\frac{\partial}{\partial t}\omega^\alpha + J(\psi^\alpha,\omega^\alpha-b^\alpha) &= -\frac{1}{2}J(h,b^\alpha),
\label{meZero-redux}\\
\omega^\alpha &= (\Delta-1) (1-\alpha \Delta )\psi^\alpha + f.
\label{constrtZero-redux}
\end{align}
Here, as before, $J(a,b)=\nabla^\perp a\cdot \nabla b=a_x b_y - b_x a_y$ denotes the Jacobian of any smooth functions $a$ and $b$ defined on the $(x,y)$ plane.


Equilibrium states of the $\alpha$-TQG system in the equations \eqref{ceZero-redux}-\eqref{constrtZero-redux} satisfy $J(\psi^\alpha_e, \omega^\alpha_e) = J(\psi^\alpha_e, b^\alpha_e)=J(h, b^\alpha_e)=0.$
The equilibrium TQG state considered in \cite{Holm2021} was given via the specification of the following
gradient fields 
\[
\begin{array}{c}
\nabla\psi^\alpha_{e}=-U\yhat,\ \nabla\omega^\alpha_{e}=(U-\beta)\yhat,\ \nabla f=-\beta\yhat\\
\\
\nabla b^\alpha_{e}=-B\yhat,\ \nabla\rmh=-H\yhat
\end{array}
\]
where we have taken $f=1-\beta y$ and the equilibrium parameters $U, \beta, B, H \in \reals$ are all constants.
% For the $\alpha$-TQG equations, we have the following specification for the $\alpha$-regularised stream function corresponding to the equilibrium state
% \[
% \nabla{\psi}^\alpha_{e}=-U\yhat.
% \]
% which follows from a particular solution to
% \[
% (1-\alpha^{2}\Delta)\nabla\tilde{\psi}_{e}=\nabla\psi_{e}.
% \]
Linearising the $\alpha$-TQG system around the steady state produces the
following evolution equations for the perturbations $\omega'$, $b'$
and ${\psi}'$
\begin{subequations}\label{eq: linear alpha tqg}
\begin{align}
\omega_{t}'+U\omega'_{x}+(U+B-\beta){\psi}_{x}' & =(U-H/2)b'_{x}
\\
b'_{t}+Ub_{x}'-B{\psi}_{x}' & =0\\
{\color{blue}\Big((1-\alpha\Delta)(1-\Delta)\Big)}{\psi}' & =-\,\omega'. \label{eq: linear alpha tqg psi}
\end{align}
\end{subequations}
Since these equations are linear with constant coefficients, one has
the plane wave solutions
\[
\omega'=e^{i(\bk\cdot\bx-\nu t)}\hat{\omega},\quad b'=e^{i(\bk\cdot\bx-\nu t)}\hat{b},\quad{\psi}'=e^{i(\bk\cdot\bx-\nu t)}\hat{{\psi}}.
\]
Further, from \eqref{eq: linear alpha tqg psi} we obtain
\[
-\,\hat{\omega}={\color{blue}(|\bk|^{2}+1)(\alpha|\bk|^{2}+1)}\hat{{\psi}}.
\]
Substituting these solutions into the linearised equations we have
\[
\begin{aligned}(\nu-kU)\hat{\omega}-k(U+B-\beta)\hat{{\psi}} & =-k(U-H/2)\hat{b}\\
\left(\nu-kU\right)\hat{b} & =-kB\hat{{\psi}}
\end{aligned}
\]
where $k$ is the first component of $\bk$.
From the above we obtain a quadratic formula for the Doppler-shifted phase speed $C = C(\alpha):=\left(\nu(\alpha)-kU\right)/k$
\[
C^{2}(|\bk|^{2}+1)(\alpha|\bk|^{2}+1)+CX+Y=0.
\]
where $X:=U+B-\beta$
and $Y:=(U-H/2)B$. Thus, the dispersion relation for the thermal Rossby wave for TQG possesses two branches, 
corresponding to two different phase velocities,
\begin{equation}\label{eq: doppler shift phase speed}
C(\alpha)=\frac{-X\pm\sqrt{X^{2}-4Y{\color{blue}(|\bk|^{2}+1)(\alpha|\bk|^{2}+1)}}}
{2{\color{blue}(|\bk|^{2}+1)(\alpha|\bk|^{2}+1)}}.
\end{equation}
% \[
% \begin{aligned}C(\alpha) & =\frac{-X\pm\sqrt{X^{2}-4Y\left(\alpha|\bk|^{4}+(1+\alpha)|\bk|^{2}+1\right)}}{2\left(\alpha|\bk|^{4}+(1+\alpha)|\bk|^{2}+1\right)}\\
%  & =-\frac{X}{2\left(\alpha|\bk|^{4}+(1+\alpha)|\bk|^{2}+1\right)}\\
%  & \qquad\pm\frac{\sqrt{X^{2}-4Y\left(\alpha|\bk|^{4}+(1+\alpha)|\bk|^{2}+1\right)}}{2\left(\alpha|\bk|^{4}+(1+\alpha)|\bk|^{2}+1\right)}\\
%  & =-\frac{X}{2\left(\alpha|\bk|^{4}+(1+\alpha)|\bk|^{2}+1\right)}\\
%  & \qquad\pm\frac{1}{2}\sqrt{\frac{1}{\left(\alpha|\bk|^{4}+(1+\alpha)|\bk|^{2}+1\right)}\left(\frac{X^{2}}{\left(\alpha|\bk|^{4}+(1+\alpha)|\bk|^{2}+1\right)}-4Y\right)}
% \end{aligned}
% \]
Upon setting $\alpha=0$ in \eqref{eq: doppler shift phase speed}, we recover the Doppler-shifted phase speed of {\color{blue}thermal Rossby waves for the TQG system in \cite{Holm2021}. When $\alpha=0$, $B=0$, and $U=0$ in \eqref{eq: doppler shift phase speed}, we recover the standard dispersion relation for QG Rossby waves in non-dimensional variables.} 

As discussed in \cite{Holm2021} for the TQG system, when $Y>0$, {\color{blue}the Doppler shifted phase velocity in \eqref{eq: doppler shift phase speed} for the linearised wave motion becomes complex at high wavenumber $|\bk| \gg 1$; namely for $(|\bk|^{2}+1)(\alpha|\bk|^{2}+1)\ge X^{2}/(4Y)$, for both branches of the dispersion relation. However, the growth-rate of the instability found from the imaginary part of $C(\alpha)$ in \eqref{eq: doppler shift phase speed} decays to zero as $O( |\bk|^{-2})$, for $|\bk|\gg1$. Indeed, the linear stability analysis leading to $C(\alpha)$ predicts that the maximum growth rate occurs at a finite wavenumber $|\bk|_{\max}$ which depends on the value of $\alpha$, beyond which the growth rate of the linearised TQG wave amplitude falls rapidly to zero. One would expect that simulated solutions of $\alpha$-TQG would be most active at the length-scale corresponding to $|\bk|_{\max}$, at which the linearised thermal Rossby waves are the most unstable}. If this maximum activity length-scale is near the grid truncation size, then numerical truncation errors could cause additional numerical stability issues! We have experience such problems during our testing of the numerical algorithm for the TQG system. Even for equilibrium solution ``sanity" check tests, we have found that unless the time step was taken to be incredibly small, high wavenumber truncation errors have caused our numerical solutions to eventually blow up.

\begin{figure}[h!]
\centering
\includegraphics[width=0.6\textwidth]{Kato Existence/growth_rate.png}
\caption{An example of the growth-rate of {\color{blue}linearised TQG waves as determined from the imaginary part of $C(\alpha)$ in equation \eqref{eq: doppler shift phase speed}}, plotted for different values of $\alpha$. We observe that increasing $\alpha$ shifts the wavenumber at the maximum growth-rate to lower values.}
\label{fig: growth rate}
\end{figure}

The magnitude of $\alpha$ {\color{blue} controls the unstable growth rate of linearised TQG waves at asymptotically high wavenumbers. That is, the presence of $\alpha$} regularises the wave activity at high wavenumbers, see Figure \ref{fig: growth rate}. Thus, from the perspective of numerics, the $\alpha$ regularisation is available to control numerical problems that may arise from the inherent model instability {\color{blue}at high wavenumbers}, without the need for additional dissipation terms in the equation.

\subsection{Numerical example}\label{sec: numerics example}
The numerical setup we consider for this paper is as follows.
The spatial domain $\domain$ is an unit square with doubly periodic boundaries.
We chose to discretise $\domain$ using a grid that 
consists of $256\times256$ cells, i.e. $\cardinality(\domain_\delta) = 256\times256$. This was the maximum resolution we could computationally afford, to obtain results over a reasonable amount of time.

We computed $\alpha$-TQG solutions for the following values of $\alpha$ -- $\frac{1}{16^{2}},\frac{1}{32^{2}},\frac{1}{64^{2}},\frac{1}{128^{2}},\frac{1}{180^{2}},\frac{1}{220^{2}},\frac{1}{256^{2}}$ and $0$.
Note when $\alpha=0$ we get the TQG system.
For all cases, the following initial conditions were used,
% \begin{subequations}
% \begin{equation}
% \begin{equations}
\begin{align}
\omega(0,x,y) & =\sin(8\pi x)\sin(8\pi y)+0.4\cos(6\pi x)\cos(6\pi y)\label{eq: pv initial condition}\\
 & \quad+0.3\cos(10\pi x)\cos(4\pi y)+0.02\sin(2\pi y)+0.02\sin(2\pi x) \nonumber \\
b(0,x,y) & =\sin(2\pi y)-1, \label{eq: buoyancy initial condition}
\end{align}
% \end{equation}
% \end{subequations}
% \end{equations}
see Figure \ref{fig: initial conditions} for illustrations,
as well as the following bathymetry and rotation fields
% \begin{equations}
\begin{align}
h(x,y) & =\cos(2\pi x)+0.5\cos(4\pi x)+\frac{1}{2}\cos(6\pi x) \label{eq: bathymetry}\\
f(x,y) & =0.4\cos(4\pi x)\cos(4\pi y). \label{eq: rotation}
\end{align}
% \end{equations}
For time stepping, we used $\Delta t = 0.0005$ in all cases to facilitate comparisons. This choice satisfies the CFL condition for the $\alpha=0$ case. 

We computed each solution for $5000$ time steps. See \cite{youtube_2021} for a video of the full simulation. Figures \ref{fig: snapshot buoyancy}, \ref{fig: snapshot pv} and \ref{fig: snapshot velocity magnitude} show $\alpha$-TQG solution snapshots of buoyancy, potential vorticity and velocity magnitude respectively, at the $1280$'th and $2600$'th time steps, for $\alpha$ values $0, \frac1{128^2}, \frac1{64^2}$ and $\frac1{16^2}$. The interpretation of the regularisation parameter $\alpha$ is that its square root value corresponds to the fraction of the domain's length scale that get regularised.
At the $1280$'th time step, the flows are in early spin-up phase.
At the $2600$'th time step, although the flows are still in spin-up phase, much more flow features have developed.
The sub-figures illustrate via comparisons, how $\alpha$ controls the development of small scale features and instabilities. Increasing $\alpha$ leads to more regularisation at larger scales.

In view of Proposition \ref{prop:alphaConv}, we investigated numerically the convergence of $\alpha$-TQG to TQG using our numerical setup. Consider the relative error between TQG buoyancy and $\alpha$-TQG buoyancy, 
\begin{align}
e_b(t, \alpha) &:= \frac{\|b(t) - b^\alpha(t)\|_{H^1}}{\|b(t)\|_{H^1}}\label{eq: relative error buoyancy}
\end{align}
and the relative error between TQG potential vorticity and $\alpha$-TQG potential vorticity,
% \begin{subequations}
\begin{align}
    e_\omega(t, \alpha) &:= \frac{\|\omega(t) - \omega^\alpha(t)\|_{L^2}}{\|\omega(t)\|_{L^2}}.\label{eq: relative error pv}
\end{align}
% \end{subequations}
% \end{equation}
The norms were chosen in view of Proposition \ref{prop:alphaConv}.
Figures \ref{fig: relative error buoyancy time series} and \ref{fig: relative error pv time series} show plots of $e_b(t, \alpha)$ and $e_\omega(t, \alpha)$
as functions of time only, for fixed $\alpha$ values $\frac{1}{16^2}, \frac{1}{32^2}, \frac1{64^2}, \frac1{128^2}$ and $\frac1{220^2}$, from the initial time up to and including the $2800$'th time step.
We observe that starting from $0$, the relative errors $e_b$ and $e_\omega$ initially increase over time but plateau at around and beyond the $2000$'th time step. 
Up to the $1400$'th time step, 
the plotted relative errors remain less than $1.0$, and are arranged in the ascending order of $\alpha$, i.e. smaller $\alpha$'s give smaller relative errors.

We note that, if we compare and contrast the relative error results with the solution snapshots of buoyancy and potential vorticity, particularly at the $2600$'th time step (shown in Figures \ref{fig: snapshot buoyancy 1.30} and \ref{fig: snapshot pv 1.30}), we observe "discrepancies" -- for lack of a better term -- between the results. For example, in Figure \ref{fig: snapshot buoyancy 1.30}, if we compare the $\alpha=\frac1{128^2}$ snapshot with the $\alpha=\frac1{16^2}$ one, the former
show small scale features that are much closer to those that exist in the reference TQG $\alpha=0$ solution. However, according to the relative error measurements, 
% especially $e_b$, 
the two regularised solutions are more or less equivalent in their differences to the reference TQG solution at time step $2600$.

If we fix the value of the time parameter in $e_b(t,\alpha)$ and $e_\omega(t, \alpha)$, and vary $\alpha$, we can estimate the convergence rate of $\alpha$-TQG to TQG for our numerical setup. Proposition \ref{prop:alphaConv} predicts a convergence rate of $1$ in $\alpha$, using the $H^1$ norm on the buoyancy differences and the $L^2$ norm on the potential vorticity differences.
Note that, in \eqref{rateOfConv}, the left hand side evaluates a supremum over a given compact time interval. We see in Figures \ref{fig: relative error buoyancy time series} and \ref{fig: relative error pv time series} that the relative errors are monotonic up to around the $1500$'th time step mark. So for a given time point $T$ between the initial time and the $1500$'th time step, we assume we can evaluate $e_b$ and $e_\omega$ at $T$ to estimate the supremum over $[0,T]$. 

Figures \ref{fig: relative error convergence buoyancy} and \ref{fig: relative error convergence pv} show plots -- in log-log scale -- of $e_b$ and $e_\omega$ as functions of $\alpha$ only at the $600$'th, $800$'th, $1000$'th and $1200$'th time steps, for all the chosen $\alpha$ values. These numbers of time steps correspond to $T=0.3$, $T=0.4$, $T=0.5$ and $T=0.6$ respectively. We also plotted in Figures \ref{fig: relative error convergence buoyancy} and \ref{fig: relative error convergence pv} linear functions of $\alpha$ to provide reference order 1 slopes.
Comparing the results to the reference, we see that the theoretical convergence rate of 1 is attained for $T=0.3$ ($600$'th time step), $T=0.4$ ($800$'th time step) and $T=0.5$ ($1000$'th time step). However for $T=0.6$ ($1200$'th time step), the convergence rates are at best order $1/2$.


% initial condition plot
\begin{figure}
\centering
\includegraphics[width=0.6\textwidth]{Kato Existence/initial_conditions_buoyancy_pv.png}
\caption{Initial conditions -- buoyancy \eqref{eq: buoyancy initial condition} on the left, and potential vorticity \eqref{eq: pv initial condition} on the right. The different colours of the PV plot correspond to positive and negative values of PV, which can be interpreted as clockwise and anticlockwise eddies respectively.}
\label{fig: initial conditions} 
\end{figure}

% show figures of solution snapshots
\begin{figure}[t]
\centering
 \begin{subfigure}[b]{0.6\textwidth}
     \centering
     \includegraphics[trim={340 25 196 5},clip,width=\textwidth]{Kato Existence/alpha_convergence_bouyancy_comparisons_t_0.64.png}
     \caption{}
     \label{fig: snapshot buoyancy 0.64}
 \end{subfigure}
 \vfill
 \begin{subfigure}[b]{0.6\textwidth}
     \centering
     \includegraphics[trim={340 25 196 5},clip, width=\textwidth]{Kato Existence/alpha_convergence_bouyancy_comparisons_t_1.30.png}
     \caption{}
     \label{fig: snapshot buoyancy 1.30}
 \end{subfigure}
 \caption{Comparisons of solution snapshots of the $\alpha$-TQG buoyancy field that correspond to four different values of $\alpha$, at two different points in time. Potential vorticity and velocity magnitude snapshots of the same solutions are shown in Figure \ref{fig: snapshot pv} and Figure \ref{fig: snapshot velocity magnitude} respectively. Shown in each sub-figure are the results corresponding to $\alpha = 0$ (top left), $\alpha = \frac1{128^2}$ (top right), $\alpha = \frac1{64^2}$ (bottom right) and $\alpha = \frac1{16^2}$ (bottom left). When $\alpha=0$, the solution is of the TQG system. Sub-figure (A) shows the solutions at the $1280$'th time step, or equivalently when $t=0.64$. Sub-figure (B) shows the solutions at the $2600$'th time step, or equivalently when $t=1.30$. The flows in both sub-figures are at different stages of spin-up, with the flow at $t=1.30$ showing more developed features. The $\alpha$ parameter is  interpreted as the fraction of the domain's length-scale squared value at which regularisation is applied. Due to regularisation, the flows do develop differently. Nevertheless, we observe that as $\alpha$ gets smaller, the $\alpha$-TQG flow features converge to that of the TQG flow.}
 \label{fig: snapshot buoyancy}
\end{figure}

\begin{figure}[t]
\centering
 \begin{subfigure}[b]{0.6\textwidth}
     \centering
     \includegraphics[trim={340 25 196 5},clip,width=\textwidth]{Kato Existence/alpha_convergence_pv_comparisons_t_0.64.png}
     \caption{}
     \label{fig: snapshot pv 0.64}
 \end{subfigure}
 \vfill
 \begin{subfigure}[b]{0.6\textwidth}
     \centering
     \includegraphics[trim={340 25 196 5},clip, width=\textwidth]{Kato Existence/alpha_convergence_pv_comparisons_t_1.30.png}
     \caption{}
     \label{fig: snapshot pv 1.30}
 \end{subfigure}
 \caption{Comparisons of solution snapshots of the $\alpha$-TQG potential vorticity field that correspond to four different values of $\alpha$, at two different points in time. See the caption of Figure \ref{fig: snapshot buoyancy} for explanations of the arrangements of these plots. Buoyancy and velocity magnitude snapshots of the same solutions are shown in Figure \ref{fig: snapshot buoyancy} and Figure \ref{fig: snapshot velocity magnitude} respectively. As in Figure \ref{fig: initial conditions}, the different colours of the PV field correspond to positive and negative values of PV, which can be interpreted as clockwise and anticlockwise eddies respectively. In sub-figure (B), we observe more clearly the regularisation effects of $\alpha$. As $\alpha$ 
 increases, the flows develop in different ways -- features at smaller scales no longer develop, and larger features evolve differently as a result.
 Nevertheless, we observe that as $\alpha$ gets smaller, the $\alpha$-TQG flow features converge to that of the TQG flow.}
 \label{fig: snapshot pv}
\end{figure}

\begin{figure}[t]
\centering
 \begin{subfigure}[b]{0.6\textwidth}
     \centering
     \includegraphics[trim={340 25 151 5},clip,width=\textwidth]{Kato Existence/alpha_convergence_velocity_comparisons_t_0.64.png}
     \caption{}
     \label{fig: snapshot velocity magnitude 0.64}
 \end{subfigure}
 \vfill
 \begin{subfigure}[b]{0.6\textwidth}
     \centering
     \includegraphics[trim={340 25 151 5},clip, width=\textwidth]{Kato Existence/alpha_convergence_velocity_comparisons_t_1.30.png}
     \caption{}
     \label{fig: snapshot velocity magnitude 1.30}
 \end{subfigure}
 \caption{Comparisons of solution snapshots of the $\alpha$-TQG velocity magnitudes that correspond to four different values of $\alpha$, at two different points in time. See the caption of Figure \ref{fig: snapshot buoyancy} for explanations of the arrangements of these plots. 
 Buoyancy and potential vorticity snapshots of the same solutions are shown in Figure \ref{fig: snapshot buoyancy} and Figure \ref{fig: snapshot pv} respectively. 
%  Here we used the Turbo colour scheme to better distinguish the different ranges of values. 
 Using the same scale for colouring, we observe in both sub-figures the strength of the colours weaken as $\alpha$ increases. This indicates smoothing of large velocity magnitudes.
 Additionally, in sub-figure (B), we observe how features at smaller scales get smoothed out. In particular, in the $\alpha=\frac1{16^2}$ plot, we see that essentially only large scale vorticies remain. Hence, considering the velocity field as a part of the system's nonlinear advection operator, these figures help us to better visualise how the flow features developed in Figure \ref{fig: snapshot buoyancy} and Figure \ref{fig: snapshot pv}. }
%  We observe that as $\alpha$ gets smaller, the $\alpha$-TQG flow features converge to that of the TQG flow. }
 \label{fig: snapshot velocity magnitude}
\end{figure}

% show figures of error convergence
\begin{figure}[t]
\centering
 \begin{subfigure}[b]{0.7\textwidth}
     \centering
     \includegraphics[width=\textwidth]{Kato Existence/relative_error_buoyancy.png}
     \caption{
    %  Plots of the bouyancy relative error function $e_b(t, \alpha)$ defined in \eqref{eq: relative error buoyancy} as a function of time only for different values of $\alpha$.
     }
     \label{fig: relative error buoyancy time series}
 \end{subfigure}
%  \hfill
 \begin{subfigure}[b]{0.7\textwidth}
     \centering
     \includegraphics[width=\textwidth]{Kato Existence/relative_error_pv.png}
     \caption{
    %  Plots of the potential vorticity relative error function $e_\omega(t, \alpha)$ defined in \eqref{eq: relative error pv} as a function of time for different values of $\alpha$.
     }
     \label{fig: relative error pv time series}
 \end{subfigure}
 \caption{Sub-figures (A) and (B) show, respectively, plots of the relative error functions $e_b(t, \alpha)$ and $e_\omega(t, \alpha)$
 as functions of time only, for the fixed $\alpha$ values $\frac{1}{16^2}$, $\frac1{32^2}$, $\frac1{64^2}$, $\frac1{128^2}$ and $\frac1{220^2}$. See equations \eqref{eq: relative error buoyancy} and \eqref{eq: relative error pv} for the definitions of $e_b$ and $e_\omega$ respectively. The plots are shown from $t=0$ up to and including $t=1.4$, which is equivalent to $2800$ time steps using $\Delta t = 0.0005$.
 We observe that, starting from $0$, all plots of  $e_b$ and $e_\omega$ increase initially, and plateau at around the $2000$'th time step. Further, up to the $1400$'th time step the plotted relative errors remain less than $1.0$ and are arranged in the ascending order of $\alpha$. Relating these relative error results at the $2600$'th time step to the solution snapshots at the same time point (shown in figures \ref{fig: snapshot buoyancy 1.30} and \ref{fig: snapshot pv 1.30}), we see that although the snapshots show convergence of flow features, the relative error values suggest all the $\alpha$-TQG solutions are more or less equally far away from the TQG flow.
 }
  \label{fig: relative errors time series}
\end{figure}

\begin{figure}[t]
\centering
 \begin{subfigure}[b]{0.7\textwidth}
     \centering
     \includegraphics[width=\textwidth]{Kato Existence/relative_error_convergency_buoyancy.png}
     \caption{}
     \label{fig: relative error convergence buoyancy}
 \end{subfigure}
%  \hfill
 \begin{subfigure}[b]{0.7\textwidth}
     \centering
     \includegraphics[width=\textwidth]{Kato Existence/relative_error_convergency_pv.png}
     \caption{}
     \label{fig: relative error convergence pv}
 \end{subfigure}
 \caption{
 Sub-figures (A) and (B) show, respectively, plots in log-log scale of the relative error functions $e_b(t, \alpha)$, and $e_\omega(t, \alpha)$
 as functions of $\alpha$ only, at the fixed time values $t=0.3$ (equivalently at the $600$'th time step), $t=0.4$ (equivalently at the $800$'th time step), $t=0.5$ (equivalently at the $1000$'th time step) and $t=0.6$ (equivalently at the $1200$'th time step). 
  In view of Proposition \ref{prop:alphaConv}, we assumed that, based on the initial monotonicity of the relative errors (see Figure \ref{fig: relative errors time series}), the supremum over $[0,T]$ in \eqref{rateOfConv} can be estimated by evaluating $e_b$ and $e_\omega$ at $T$.
 Proposition \ref{prop:alphaConv} predicts that up to a certain time, the rate of convergence of $e_b$ and $e_\omega$ to $0$ should be no less than order 1 in $\alpha$.
 In both sub-figures we have plotted, as the reference for comparison, linear functions of  $\alpha$. Thus, comparing slopes to the reference, we see that numerically we get order $1$ convergence for $t=0.3$, $t=0.4$ and $t=0.5$. However, for $t=0.6$, the rate of convergence is no more than $1/2$.
 }
\end{figure}


% show figures of errors in spectral space
